Understanding the Role of Feedback in Online Learning with Switching Costs

In this paper, we study the role of feedback in online learning with switching costs. It has been shown that the minimax regret is $\widetilde{\Theta}(T^{2/3})$ under bandit feedback and improves to $\widetilde{\Theta}(\sqrt{T})$ under full-information feedback, where $T$ is the length of the time horizon. However, it remains largely unknown how the amount and type of feedback generally impact regret. To this end, we first consider the setting of bandit learning with extra observations; that is, in addition to the typical bandit feedback, the learner can freely make a total of $B_{\mathrm{ex}}$ extra observations. We fully characterize the minimax regret in this setting, which exhibits an interesting phase-transition phenomenon: when $B_{\mathrm{ex}} = O(T^{2/3})$, the regret remains $\widetilde{\Theta}(T^{2/3})$, but when $B_{\mathrm{ex}} = \Omega(T^{2/3})$, it becomes $\widetilde{\Theta}(T/\sqrt{B_{\mathrm{ex}}})$, which improves as the budget $B_{\mathrm{ex}}$ increases. To design algorithms that can achieve the minimax regret, it is instructive to consider a more general setting where the learner has a budget of $B$ total observations. We fully characterize the minimax regret in this setting as well and show that it is $\widetilde{\Theta}(T/\sqrt{B})$, which scales smoothly with the total budget $B$. Furthermore, we propose a generic algorithmic framework, which enables us to design different learning algorithms that can achieve matching upper bounds for both settings based on the amount and type of feedback. One interesting finding is that while bandit feedback can still guarantee optimal regret when the budget is relatively limited, it no longer suffices to achieve optimal regret when the budget is relatively large.

==> app_duo.tex <==
\newpage

\appendix
\onecolumn

\section{More Discussion on Related Work}\label{app:purdue_difference}

\bo{This section needs to be reorganized later; it should probably be Appendix A or B, depending the order in which it is referred to}\duo{now the sections in appendix should be in correct order}\bo{This section still needs to be reorganized. Shi's work should belong to one of the categories as well. Think about a logical order of different topics here, rather than just a list of topics}\duo{I've changed the order but I don't think Shi's paper is one of them as they formulate a new problem.}

In this section, we first elaborate on \citet{shi2022power} to show the difference between their work and ours. Generally speaking, their problem setup as well as the regret definition are both completely different from ours.

In particular, their loss is defined as:
\begin{equation}\label{eqn:purdue_cost_def}
\operatorname{Cost}(1: T) := \sum_{t=1}^T\left\{\ell_t[X_t] + \beta_1 \sum_{k \in \mathcal{K}(t)} \mathbb{I}_{\{k \notin \mathcal{K}(t-1)\}}+\beta_2 z(t)\right\},
\end{equation}
where $\{\mathcal{K}(t)\}_{t=1}^T$ is a sequence of action sets with cardinality $m\in [K]$ and $z(t)\in\{0,1\}$ indicates whether the learner asks for full feedback at round $t$. Moreover, at each round, the learner should first determine the set $\mathcal{K}(t)$, and then the decision $X_t$ can be made \emph{only from} this set. By the end of each round, the loss of all actions in $\mathcal{K}(t)$ will be revealed to the learner. The second term in Eq. (\ref{eqn:purdue_cost_def}) could be viewed as ``switching costs'' in their definition, which is roughly the total variation on set $\mathcal{K}(t)$ throughout the game. The last term indicates that whenever the learner asks for full feedback, she also needs to pay for some cost $\beta_2$.

However, when $m=1$, their switching cost definition reduces to the standard one. Furthermore, the $\wtTheta(T^{2/3})$ optimal regret they show when $m=1$, implies that, full information from $\wtTheta(T^{2/3})$ rounds does not improve the optimal regret rate in the bandit setting, which is just a special case of our Theorem~\ref{thm:bandit_extra_minimax} when $\Bex=\wtTheta(T^{2/3})$.

In the rest of this section, we present more detailed discussion on related work.

\textbf{Online Learning with Total Observation Budget.} \citet{seldin2014prediction} also considers total observation budget in the context of online learning, where the learner can freely request feedback, as long as the total amount does not exceed the given total budget, \emph{but without out switching costs.} With this key difference, we need to take switching costs into account in both lower bound analysis as well as the algorithm design on top of their work.

\textbf{Bandit and Expert Problems with Switching Costs.}
Minimax optimal regrets with switching costs under bandit and full-information feedback over a finite action set have been well studied. In the bandit setting, the optimal regret is $\widetilde{\Theta}(\PTP)$. Specifically, \citet{dekel2014bandits} shows a lower bound by constructing a loss sequence via a multi-scale random walk, and one simple way to obtain a matching upper bound (up to logarithmic factors) is a batched version~\citep{Dekel2012OnlineBL} of the EXP3 algorithm~\citep{auer2002nonstochastic}. In the expert setting, the optimal regret is $\widetilde{\Theta}(\sqrt{T \ln K})$, which can be achieved by multiple algorithms including Shrinking Dartboard (SD)~\citep{geulen2010regret} and Follow-the-Perturbed-Leader (FTPL)~\citep{devroye2013prediction}. Our work studies a more general setting where there is a total observation budget, but the type of feedback can be quite flexible. This setting includes the bandit and expert problems as two special cases. 

\textbf{Online Learning with Switching Costs and Feedback Graphs.}
In this setting, while switching costs are added to the learner's loss, the learner also receives some additional observations besides bandit feedback at each round, which is close to the setting we consider. Particularly, given a feedback graph $G$, the learner observes the loss of the neighbors of the action (including the action itself)
%\duo{I need to double check. It's related to so-called weakly/strongly-observable graph} \bo{I checked \citep[the second last paragraph of Section 2]{arora2019bandits}.}
she plays. However, the feedback graph is given and is \emph{not} of the learner's choice. In this setting, the optimal regret is $\wtTheta(\gamma(G)^{1/3} T^{2/3})$~\citep{arora2019bandits}, where $\gamma(G)$ is the domination number of feedback graph $G$. That is, in the worst case one still cannot improve the regret with respect to $T$ compared to the bandit setting. On the contrary, in the setting we consider, the learner can freely decide the loss of which actions to observe at each round, which leads to different (and more interesting) regret bounds.

\textbf{Online Learning against Adaptive Adversaries}. Online learning with switching costs can also be viewed as a special case of \emph{learning against adaptive adversaries}, where the losses at round $t$ are adapted to actions taken at both rounds $t$ and $t-1$. Such adversaries have a \emph{bounded memory} (of size one in this case), in the sense that they could adapt only up to the \emph{most recent} actions, instead of any history in the earlier rounds \citep{cesa2013online}. Using the multi-scale random walk argument~\citep{dekel2014bandits} as a building block, it has been shown that against \emph{adaptive adversaries with a memory of size one}, the minimax-optimal \emph{policy regret} is $\wtTheta(T^{2/3})$ under \emph{both} bandit feedback~\citep{cesa2013online} and full-information feedback~\citep{feng2018online}.
This is fundamentally different from the special case with switching costs, where there is a gap in the optimal regret ($\wtTheta(T^{2/3})$ in bandit feedback vs. $\Theta(\sqrt{T})$ in full-formation feedback).

\textbf{Online Learning with Limited Switches.}
In this line of work, in contrast to the switching-cost settings above, the learner does not get penalized for making switches, but the total number of switches throughout the game is limited (e.g., capped at $S$)~\citep{altschuler2018online}. Compared to our setting, a key difference is that there, switching is a constraint rather than a penalization added to the total loss. 
%\citet{altschuler2018online} exploits this setting by considering that $S$ is a hard cap on total number of switches. 
In the bandit setting, the optimal regret is $\widetilde{\Theta}(T\sqrt{K/S})$, i.e., a larger switching budget helps improve the regret.
In the expert setting, however, there is a phase-transition phenomenon: while the optimal regret is $\wtTheta(T \ln{K} / S)$ when $S=O(\sqrt{T \ln{K}})$, it remains $\wtTheta(\sqrt{T \ln{K}})$ when $S=\Omega(\sqrt{T \ln{K}})$.
%\bo{I think it is fine to use $S$ here as it is also the number of switches}\duo{I think you are right}
%\bo{Shouldn't the range of $S$ be switched? Can you double check?}\duo{when $S$ is large, it doesn't affect the regret, otherwise it increases the regret, right? I think it's correct after checking the 2018 COLT paper.}\bo{thanks for checking.}





\section{A Motivating Example of Learning with Total Observation Budget}\label{app:motivate}
A motivating example for our extra observations within a total budget is from edge computing  \citep{Murshed2019MachineLA, shi2022power}: say each time an image is delivered to an edge serving for processing (e.g., classification \citep{He2015DelvingDI}, denoising \citep{Buades2005ARO}). There are $K$ Machine Learning (ML) to choose from, which however are stored in the remote could and cannot be simultaneously deployed at the edge server due to its limited capacity. After each round the edge processes the image using the chosen ML model, the performance (e.g., accuracy) of this model is revealed. Additionally, we could also evaluate the same image at other ML models, for which however we need to transmit ML models between cloud and edge server through wireless channels, thus suffering latency/computation resources overhead \citep{Elbamby2019WirelessEC}. Because of that, although we could make observations from any other actions at our own choice, we may want to limit the total number of them to avoid significant overhead.
\section{Proof of Proposition \ref{prop:bandit_extra_lower_bound}}\label{app:extra_lower_bound_proof}
\begin{proof}[Proof of Proposition \ref{prop:bandit_extra_lower_bound}]
Our proof is built on the Yao's minimax principle \cite{yao1977crobabilistic}. That is to say, we are going to establish a lower bound on the expected regret for any deterministic learner over a class of randomly generated loss sequences, and that would further imply the same lower bound for any randomized learner over some loss sequence in this class .

%\bo{Recall important notations here.}
The instance construction we adopt will be exactly the same from algorithm 1 in \citet{shi2022power}, but with some differences in the analysis. For convenience we provide its pseudo-code in Algorithm \ref{alg:purdue_instance} and let $\mathcal{N}(0,\sigma^2)$ denotes Gaussian distribution with mean zero and variance $\sigma^2$.

\begin{algorithm}[h]
    \caption{Loss Generation from \citet{shi2022power}} 
    \label{alg:purdue_instance}
    \begin{algorithmic}[1]
        \STATE \textbf{Input:} optimality gap $\epsilon$ and noise variance $\sigma^2$
        \STATE \textbf{Initialization:} choose the identity of optimal action $k^*$ uniformly at random from $[K]$; Gaussian process $G(t)=0, \forall t\geq 0$; define functions $\delta(t):=\max\{i\geq 0:2^i \text{~divides~}t\}$ and  $\rho(t):=t-2^{\delta(t)}, \forall t\geq 0$
        
        \FOR {time $1 = 1: T$}
            \STATE $G(t)=G(\rho(t))+\xi(t)$, where each $\xi(t)$ is an i.i.d sample from $\mathcal{N}(0,\sigma^2)$
            \STATE $\ell_t^{\mathrm{init}}[k] = G(t)-\epsilon\cdot \bI_{\{k=k^*\}}+\gamma_k(t),\forall k \in[K]$, where each $\gamma_k(t)$ is an i.i.d sample from $\mathcal{N}(0,\sigma^2)$
            \STATE $\ell_t[k] = \min_{x\in[0,1]}|x-\ell_t^{\mathrm{init}}[k]|, \forall k\in[K]$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

We first give some additional notations needed for this proof following \citet{shi2022power}. For $k\in[K]$, $\bP_{k}$ denotes the conditional probability measure given the optimal action $k^{*}=k$, i.e., $\bP_{k}(\cdot):= \bP(\cdot |k^{*}=k)$. As a special case, when $k^*=0$,  $\bP_{0}$ denotes the conditional probability measure when all the arms are identical and there is no special arm. $\bE_{k}[\cdot]:=\bE[\cdot|k^*=k]$ denotes the conditional expectation under measure $\bP_{k}$ and $\bE[\cdot]:=\frac{1}{K}\sum_{k=1}^K\bE_{k}[\cdot]$. $\ell^{\mathrm{ob}}(1: T)$ denotes the observed loss sequence throughout the game. For two probability distributions $\mathcal{P}$ and $\mathcal{Q}$, $D_{\mathrm{KL}}:=\bE_{x\sim \mathcal{P}}[\log \left(d\mathcal{P}(x)/d\mathcal{Q}(x)\right)]$ denotes the Kullback-Leibler (KL) divergence (i.e., relative
entropy) between $\mathcal{P}$ and $\mathcal{Q}$.

Let $S_t^{k}:= \bI_{\{X_{\rho(t)} = k, X_t \neq k\}} + \bI_{\{X_{\rho(t)} \neq k, X_t = k\}}$, i.e., the indicator of whether the action is switched from or to $k$ between time slot $\rho(t)$ and $t$. Let $\bar{S}^{k} := \sum_{t=1}^T S_t^{k}$, i.e., the total number of times the learner switches from or to action $k$. $\bar{S}$ denotes the total number of switches made by the learner, i.e., $\bar{S}:=\sum_{t=1}^T\bI_{\{X_t\neq X_{t-1}\}}=\sum_{k=1}^K \bar{S}^{k}/2$. Let $N_{\mathrm{extra}}^t$ be the number of extra observations made at round $t$. Naturally we have $N_{\mathrm{extra}}^t\in[0,K-1]$ and thus $\Bex \geq \sum_{t=1}^T N_{\mathrm{extra}}^t$.

According to the Appendix B in \citet{shi2022power}, for any $k \in [K]$, we have
\begin{align}
&D_{\mathrm{KL}}\left(\bP_0\left(l^{\mathrm{ob}}(1: T)\right) \| \bP_{k}\left(l^{\mathrm{ob}}(1: T)\right)\right) \nonumber\\
&\leq \sum_{t=1}^T\left[\bP_0\left(N_{\mathrm{extra}}^t=0, S_t^{k}=1\right) \cdot \frac{\epsilon^2}{2 \sigma^2}\right. \nonumber\\
&\quad + \sum_{j=1}^{K-1} \bP_0 \left(N_{\mathrm{extra}}^t=j, S_t^{k}=0, X_t \neq k\right) \cdot \frac{\epsilon^2}{2 \sigma^2} \nonumber\\
&\quad + \sum_{j=1}^{K-1} \bP_0 \left(N_{\mathrm{extra}}^t=j, S_t^{k}=0, X_t=k\right) \cdot \frac{j \epsilon^2}{2 \sigma^2} \nonumber \\
&\quad + \sum_{j=1}^{K-1} \bP_0 \left(N_{\mathrm{extra}}^t=j, S_t^{k}=1, X_t \neq k\right) \cdot \frac{2\epsilon^2}{2 \sigma^2} \nonumber \\
&\left.\quad + ~ \sum_{j=1}^{K-1} \bP_0\left(N_{\mathrm{extra}}^t=j, S_t^{k}=1, X_t=k\right) \cdot \frac{(j+1) \epsilon^2}{2 \sigma^2}\right]  \\
&\leq \sum_{t=1}^T\left[\bP_0\left(S_t^{k}=1\right) \cdot \frac{\epsilon^2}{2 \sigma^2} + \sum_{j=1}^{K-1} \bP_0 \left(N_{\mathrm{extra}}^t=j\right) \cdot \frac{j\epsilon^2}{ \sigma^2} \right]\label{eqn:6_1} \\
&\leq \log _2 T \cdot \frac{\epsilon^2}{2\sigma^2} \cdot \left( \bE_{0}\left[\bar{S}^{k}\right] + 2 \cdot \Bex\right), \label{eqn:6_2}
\end{align}
where Eq. (\ref{eqn:6_1}) is from $2 \leq j+1 \leq 2j, \forall j \geq 1$ and $\sum_{j=1}^{K-1} \bP_0(N_{\mathrm{extra}}^t = j)\cdot j = \bE_{0}\left[N_{\mathrm{extra}}^t\right]$. Eq. (\ref{eqn:6_2}) follows Lemma 3 in \citet{dekel2014bandits} and upper bounding $\sum_{t=1}^T \bE_{0}\left[N_{\mathrm{extra}}^t\right]$ by $\Bex$, since the learner makes no more than $\Bex$ extra observations. Furthermore, we have
\begin{align}
&\frac{1}{K} \sum_{k=1}^K D_{\mathrm{KL}} \left(\bP_0\left(l^{\mathrm{ob}}(1: T)\right) \| \bP_{k}\left(l^{\mathrm{ob}}(1: T)\right)\right) \nonumber \\
&\leq \frac{1}{K} \sum_{k = 1}^K \sqrt{\frac{\ln 2}{2}} \sqrt{D_{\mathrm{KL}}\left(\bP_0\left(l^{\mathrm{ob}}(1: T)\right) \| \bP_{k}\left(l^{\mathrm{ob}}(1: T)\right)\right)}\label{eqn:6_5}\\
&\leq \sqrt{\frac{\ln 2}{2}}\sqrt{\log _2 T \cdot \frac{\epsilon^2}{2\sigma^2}} \sum_{k = 1}^K \frac{1}{K}\sqrt{\bE_{0}\left[\bar{S}^{k}\right] + 2 \cdot \Bex} \\
&\leq \sqrt{\frac{\ln 2}{2}}\sqrt{\log _2 T \cdot \frac{\epsilon^2}{2\sigma^2}} \sqrt{\sum_{k = 1}^K \frac{1}{K} \left( \bE_{0}\left[\bar{S}^{k}\right] + 2 \cdot \Bex \right)} \label{eqn:6_6} \\
& = \sqrt{\frac{\ln 2}{2}}\sqrt{\log _2 T \cdot \frac{\epsilon^2}{2\sigma^2}} \sqrt{ \frac{1}{K} \left(2\cdot \bE_{0}\left[\bar{S}\right] + 2 \cdot \Bex \right)} \\
&= \frac{\epsilon}{\sigma}\sqrt{\frac{\ln 2}{2}}\sqrt{\frac{\log _2 T}{K}} \sqrt{  \left(\bE_{0}\left[\bar{S}\right] + \Bex \right)}.\label{eqn:6_7}
\end{align}
Eq. (\ref{eqn:6_5}) is from Pinsker's inequality. Eq. (\ref{eqn:6_6}) follows Jensen's inequality. Eq. (\ref{eqn:6_7}) is due to the fact that $\sum_{k = 1}^K \bE_{0}\left[\bar{S}^{k}\right] = 2\bE_{0}\left[\bar{S}\right]$.

Let $N_k$ be the number of times action $k$ is played up to round $T$. We first assume that the deterministic learner makes at most $\epsilon T$ switches, and later we will relax this assumption. In this case, we have
\begin{align}
\bE_{0}\left[\bar{S}\right] - \bE\left[\bar{S}\right] &\leq \frac{\epsilon T}{K} \sum_{k=1}^K D_{\mathrm{KL}} \left(\bP_0\left(l^{\mathrm{ob}}(1: T)\right) \| \bP_{k}\left(l^{\mathrm{ob}}(1: T)\right)\right),\\
\sum_{k=1}^K \bE_{k}[N_k] &\leq T + T\sum_{k=1}^K D_{\mathrm{KL}} \left(\bP_0\left(l^{\mathrm{ob}}(1: T)\right) \| \bP_{k}\left(l^{\mathrm{ob}}(1: T)\right)\right),
\end{align}
which follows the proof of Lemma 2 and Theorem 2 in \citet{dekel2014bandits}.

Now, we can lower bound the regret as
\begin{align}
\bE\left[R_T^{\mathrm{init}}\right] &= \frac{1}{K} \sum_{k=1}^K \bE \left[\epsilon(T-N_k) + \bar{S}|k^* = k \right] \\
&= \epsilon T - \frac{\epsilon}{K}\sum_{k=1}^K \bE_{k}\left[{N}_{k}\right] + \bE \left[\bar{S}\right] \\
& \geq \epsilon T - \frac{\epsilon T}{K} - \frac{2\epsilon T}{K} \sum_{k=1}^K D_{\mathrm{KL}} \left(\bP_0\left(l^{\mathrm{ob}}(1: T)\right) \| \bP_{k^*}\left(l^{\mathrm{ob}}(1: T)\right)\right) + \bE_{0} [\bar{S}] \\
&\geq \frac{\epsilon T}{2} - \frac{\sqrt{2\ln 2} \cdot \epsilon^2 T  \sqrt{\log _2 T} }{\sigma\sqrt{K}}  \sqrt{ \bE_{0}\left[\bar{S}\right] + \Bex} + \bE _{\bP_0}\left[\bar{S}\right]\\
&\geq \frac{\epsilon T}{2} - \frac{\sqrt{2\ln 2} \cdot \epsilon^2 T  \sqrt{\log _2 T} }{\sigma\sqrt{K}} \left( \sqrt{ \bE_{0}\left[\bar{S}\right]} +  \sqrt{ \Bex}\right) + \bE _{\bP_0}\left[\bar{S}\right] \label{eqn:6_3} \\
&\geq \frac{\epsilon T}{2} - \frac{\ln 2 \cdot   \epsilon^4 T^2  \log_2 T}{2 K \sigma^2} - \frac{ \sqrt{2 \ln 2} \cdot \epsilon^2 T \sqrt{\log_2 T} }{\sigma \sqrt{K}}  \sqrt{\Bex}. \label{eqn:6_4}
\end{align}

Eq. (\ref{eqn:6_3}) follows elementary inequality $ \sqrt{x} + \sqrt{y} \geq \sqrt{x+y}, \forall x,y\geq0$. Eq. (\ref{eqn:6_4}) is obtained by minimizing the quadratic function w.r.t. $\sqrt{ \bE_{0}\left[\bar{S}\right]}$. 

Let $R_T$ be the regret after all losses are clipped to $[0,1]$, and $R_T^{\mathrm{init}}$ be the regret before clipping over the \emph{same action sequence}. By Lemma 4 in \citet{dekel2014bandits}, if $\epsilon < 1/6$ and $\sigma = 1/(9\log_2 T)$, we have $\ex{R_T^{\mathrm{init}}}-\ex{R_T}\leq \frac{\epsilon T}{6}$. We will first assume this is true and at last verify if $\epsilon$ by our selection indeed satisfies this condition. Then by selecting $\sigma = 1/(9\log_2 T)$, we have
\begin{align}
\ex{R_T} &\geq \frac{\epsilon T}{3} - \frac{\ln 2 \cdot   \epsilon^4 T^2  \log_2 T}{2 K \sigma^2} - \frac{ \sqrt{2 \ln 2} \cdot \epsilon^2 T \sqrt{\log _2 T} }{\sigma \sqrt{K}}  \sqrt{  \Bex}\\
&\geq \frac{\epsilon T}{3} - \frac{81 \cdot   \epsilon^4 T^2  \log_2^3 T}{2 K } - \frac{ 9\sqrt{2} \cdot \epsilon^2 T \log_2^{3/2} T }{\sqrt{K}}  \sqrt{  \Bex}.
\end{align}

When $\sqrt{\Bex} \leq c_1 \frac{K^{1/6}T^{1/3}}{ \log_2^{1/2} T}$ for some $c_1>0$, we have
\begin{align}
\ex{R_T} &\geq \frac{\epsilon T}{3} - \frac{81 \cdot   \epsilon^4 T^2  \log_2^3 T}{2 K } - \frac{18 c_1 \cdot \epsilon^2 T \log_2^{3/2} T}{ \sqrt{K}}  \cdot \frac{K^{1/6}T^{1/3}}{ \log_2^{1/2} T} \\
&= \left(\frac{c_2}{3} - \frac{81c_2^4}{2} - 18c_1 c_2^2\right) \frac{K^{1/3} T^{2/3}}{18 \log_2 T} \\
&= \widetilde{\Omega}(K^{1/3}T^{2/3}).
\end{align}
The first equality is obtained by selecting $\epsilon = c_2\frac{K^{1/3}}{ T^{1/3} \log_2 T}$, where $c_2>0$ satisfies $\frac{1}{3} - \frac{81c_2^3}{2} - 18c_1 c_2 >0$.

On the other side, when $\sqrt{\Bex} > c_1 \frac{K^{1/6}T^{1/3}}{\log_2^{1/2} T}$, we have
\begin{align}
\ex{R_T} &\geq \frac{\epsilon T}{3} - \frac{81 \epsilon^4 T^2  \log_2^3 T}{2 K } \cdot \frac{ \log_2^{1/2} T}{c_1 K^{1/6}T^{1/3}} \sqrt{\Bex} - \frac{ 9\sqrt{2} \cdot \epsilon^2 T \log_2^{3/2} T}{\sqrt{K}}  \sqrt{\Bex}\label{eqn:4_5}\\
&= \frac{\epsilon T}{3} - \frac{81 \epsilon^4 T^{5/6}  \log_2^{7/2} T}{2c_1 K^{7/6} } \sqrt{\Bex} - \frac{ 9\sqrt{2} \cdot \epsilon^2 T \log_2^{3/2} T}{\sqrt{K}}  \sqrt{\Bex}\\
&= \frac{c_3 T\sqrt{K}}{3 \log_2^{3/2} T \sqrt{\Bex}} - \frac{81 c_3^4 K^{5/6} T^{5/6}}{2c_1\log_2^{5/2} T \cdot (\Bex)^{3/2}} - \frac{9 c_3^2 \sqrt{2}\sqrt{K} T }{\log_2^{3/2} T \cdot \sqrt{\Bex}}\label{eqn:4_6} \\
& \geq \frac{c_3 T\sqrt{K}}{3 \log_2^{3/2} T \sqrt{\Bex}} - \frac{81 c_3^4 \sqrt{K} T^{1/6} }{2c_1^3 \log_2^{3/2} T \cdot \sqrt{\Bex}} - \frac{9 c_3^2 \sqrt{2}\sqrt{K} T }{\log_2^{3/2} T \cdot \sqrt{\Bex}} \label{eqn:4_7} \\
&\geq \left( \frac{c_3}{3} - \frac{81c_3^4}{2c_1^3} - 18 c_3^2 \right)\frac{\sqrt{K} T }{\log_2^{3/2} T \cdot \sqrt{\Bex}}\\
&= \widetilde{\Omega}\left(T\frac{\sqrt{K} }{\sqrt{\Bex}}\right).\label{eqn:4_8}
\end{align}
Eq. (\ref{eqn:4_5}) is simply because $\frac{\log_2^{1/2} T}{c_1 K^{1/6}T^{1/3}} \sqrt{\Bex} > 1$. Eq. (\ref{eqn:4_6}) is obtained by selecting $\epsilon =\frac{c_3\sqrt{K}}{\log_2^{3/2} T \cdot \sqrt{\Bex}}$, where $c_3>0$ satisfies $ \frac{1}{3} - \frac{81{c_3}^3}{2c_1^3} - 18 c_3 > 0$. Eq. (\ref{eqn:4_7}) uses $\frac{\log_2^{1/2} T}{c_1 K^{1/6}T^{1/3}} \sqrt{\Bex} > 1$ again on the second term.
 Since $K\leq T$,  in both cases, for sufficiently large $T$, $\epsilon$ will be no greater than 1/6.

To relax the assumption we made above (i.e., the deterministic player makes no more that $\epsilon T$ switches), according to the proof of Theorem 2 in \citet{dekel2014bandits}, if the learner makes more than $\epsilon T$ switches, her regret could be lower bounded by $2R_T$, and thus the asymptotic order stays the same.

So far, we have shown an lower bound for any deterministic learner. Applying Yao's principle completes the proof. 
\end{proof}
\section{Handling Integrality Issues}\label{app:integer}
In the main body, we ignore all the integrality-related issues. In this section we show one option to solve them to make our algorithm practical while we still enjoy the same regret guarantee (order-wise). In particular, we need to run our algorithm while both batch size $\tau$ and the number of batches $N$ are integers. It suffices to show the case for $\pi_{\mathrm{flex}}$ in Proposition \ref{prop:flex upper bound} when $B<T$ as the extensions to other cases follow the same procedure.

 Recall that now we have $N=B/M$ and $\tau = T/N=MT/B$. Now define $\tau^{\prime}:=\lceil \tau \rceil = \lceil T/N \rceil = \lceil MT/B \rceil$ and $N_1$ be the largest integer $N'$ such that $N'\cdot \tau^{\prime}\leq T$. Also let $T^{\prime}:=N_1 \cdot \tau^{\prime}$. Now according to the proof of Proposition \ref{prop:flex upper bound}, over the first $T^{\prime}$ time slots, we can enjoy regret $R_{T^{\prime}}^{\pi_{\mathrm{flex}}}=O(\tau^{\prime}\sqrt{\frac{T'K\ln K}{\tau' M}})$, with batch size $\tau^{\prime}$ and number of batches $N_1$, which are now both integers. We can show the following upper bound on $R_{T^{\prime}}^{\pi_{\mathrm{flex}}}$:
\begin{align}
    R_{T^{\prime}}^{\pi_{\mathrm{flex}}} &= \sqrt{\lceil \frac{MT}{B} \rceil \frac{T^{\prime} K \ln K}{M}} \\
     &\leq  \sqrt{ \frac{2MT}{B} \cdot  \frac{T^{\prime} K \ln K}{M}} \\
     &=O(T\sqrt{\frac{K\ln K}{B}}).
\end{align}
The inequality is due to $MT\geq B$ and at the last equality we upper bound $T'$ by $T$. So far, the total number of observations we consume is $N_1 M$, which is no larger than $NM$ and hence we don't exceed the budget $B$.

For the remaining $(T-T^{\prime})$ time slots, we can just keep playing any fixed action (and do not need any feedback), which incurs $O(T-T^{\prime})=O(\tau^{\prime}) = O(MT/B)=O(T\sqrt{\frac{K\ln K}{B}})$ regret. The last equality is simply because $B\geq K\geq M$.

\section{Proof of Proposition \ref{prop:uniform_alg_upper_bound}}\label{app:uniform_alg_upper_bound_proof}
Before showing Proposition \ref{prop:uniform_alg_upper_bound}, we first need two lemmas on the properties of SD, both from \citet{geulen2010regret}.
\begin{lemma}\citep[Lemma~1]{geulen2010regret}\label{lem:SD_regret}
For \algref{framework} with any $\eta>0$, $ N\geq 1$, $I_{SD} = 1$, $\mathcal{O}_{u_b} = [K]$ and $\widehat{\ell}_b = \ell_{u_b}$  over any loss sequence, we have $\bP\left( A_b = i\right) = \bE[w_b[i]], ~\forall i\in [K] , ~b \in [N]$.
\end{lemma}

\begin{proof}[Proof of \lemref{SD_regret}]
First, in this case, we observe that in \algref{framework}, the feedback depends on the randomly chosen $u_b$ only, and thus is independent of what action is taken by the learner throughout the game. Because of that, we can fix the whole sequence $\widehat{\ell}_{1:N}$ even before the game starts.

In the following, we will show by induction that conditioning on any random feedback sequence $\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{N}= \ell_{N}^{\prime}$, $\bP\left( A_b = i|\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{N}= \ell_{N}^{\prime}  \right) = w_b[i], ~\forall i \in [K] , ~b \in [N]$.
%\xingyu{we can try to add $\omega$ into $A_b$ and $w_b$, something like $A_b^{\omega}$ and $w_b^{\omega}$. Then, for each realization of $\widehat{\ell}$, we basically say for any $\omega$.}\duo{I'm not familiar with such notation. Any reference on this?}

% \xingyu{More on the above Lemma 1: It seems to me that if we have Lemma~\ref{lem:SD_regret} as stated above (i.e., expectation on the RHS), we may not be able to establish the required result. The key is to show that $\ex{\ell_i(A_b))} = \ex{\inner{w_b}{\ell_i}}$. Then, Let first see what is corresponding part in SD paper. In particular, $\ex{\ell_i(A_b)} = \sum_k \prob{A_b = k} \ell_i[k] = \inner{w_b}{\ell_i}$, where we have used $\prob{A_b = k} = w_b$ in the SD paper. Then, we use the OMD bound for the term $\inner{w_b}{\ell_i}$.

% Now, for our case, we have 
% \begin{align}
%     \ex{\ell_i(A_b)} = \ex{\ex{\ell_i(A_b)| \widehat{\ell}_{b\ge 1}}} = \ex{ \sum_k \prob{A_b = k | \widehat{\ell}_{b\ge 1}}\ell_i(k) }
% \end{align}
% } 

The base case when $b=1$ is obviously true from the algorithm. In the following let us move to the general case when $b\geq2$:

\begin{align}
    &\bP\left( A_b = i | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{N}= \ell_{N}^{\prime}\right) \\
    =&~ W_b[i]/ W_{b-1}[i] \cdot \bP\left(\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{N}= \ell_{N}^{\prime}\right) \nonumber \\
    &+ \sum_{k=1}^K \left( 1-W_b[k]/ W_{b-1}[k] \right) \cdot w_b[i] \cdot \bP\left( A_{b-1} = k | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{N}= \ell_{N}^{\prime}\right) \label{eqn:1_1} \\
    =&~W_b[i]/ W_{b-1}[i] \cdot w_{b-1}[i] + w_b[i] \cdot \sum_{k=1}^K \left( 1-W_b[k]/ W_{b-1}[k] \right) \cdot w_{b-1}[k]  \label{eqn:1_2} \\
    =&~\frac{W_b[i]}{W_{b-1}[i]}  \cdot \frac{W_{b-1}[i]}{\sum_{j=1}^K {W_{b-1}[j]}} + \frac{W_{b}[i]}{\sum_{j=1}^K {W_{b}[j]}} \cdot \sum_{k=1}^K \left( \frac{W_{b-1}[k] - W_b[k]}{W_{b-1}[k]} \right) \cdot \frac{w_{b-1}[k]}{\sum_{j=1}^K {W_{b-1}[j]}} \\
    =&~\frac{W_b[i]}{\sum_{j=1}^K {W_{b-1}[j]}} + \frac{W_{b}[i]}{\sum_{j=1}^K {W_{b}[j]}} \cdot  \frac{\sum_{j=1}^K {W_{b-1}[j]} - \sum_{j=1}^K {W_{b}[j]}}{\sum_{j=1}^K {W_{b-1}[j]}} \\
    =&~w_b[i] \cdot \frac{\sum_{j=1}^K {W_{b}[j]}}{\sum_{j=1}^K {W_{b-1}[j]}} + w_b[i] \cdot \left(1-\frac{\sum_{j=1}^K {W_b[j]}}{\sum_{j=1}^K {W_{b-1}[j]}}\right) \\
    =&~w_b[i].
\end{align}

Eq. (\ref{eqn:1_1}) is from Line \ref{line:next_decision} in Algorithm \ref{alg:framework}. To be specific, there are two disjoint cases in which action $i$ can be played in batch $b$. One is that, $i$ is played in batch $b-1$ and it does not change according to probability $p_b$\duo{no $p_b$ any more}, and the other is that whichever action is played in batch $b-1$, action $i$ is selected from fresh randomness. (\ref{eqn:1_2}) is due to our induction. Finally, taking expectation on both sides ends the proof.
\end{proof}
Lemma \ref{lem:SD_regret} indicates that, SD does not change the marginal distribution of action selection, hence we enjoy the same regret guarantee from standard OMD (without SD).
\begin{lemma}\citep[Lemma~2]{geulen2010regret}\label{lem:SD_switch}
Running \algref{framework} as specified in Lemma~\ref{lem:SD_regret}, the expected number of switches satisfies that $\bE \left[\sum_{t=1}^T \bI\{X_{t} \neq X_{t-1}\} \right]\leq \eta N = \eta T/\tau$.
\end{lemma}
\begin{proof}[Proof of \lemref{SD_switch}]
Following the definitions, we have
\begin{align}
\bE \left[\sum_{t=1}^T \bI_{\{X_{t} \neq X_{t-1}\}} \right] &= \bE \left[ \sum_{b=2}^{N} \bI_{\{A_{b} \neq A_{b-1}\}} \right]\label{eqn:2_1}\\
    &= \sum_{b=2}^{N} \bE \left[ \bE \left[ \bI_{\{A_{b} \neq A_{b-1}\}} |\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime}, A_{b-1} = j \right] \right]\\
    &{\leq}~  \sum_{b=2}^{N}  \bE \left[1 - \exp(-\eta \cdot \widehat{\ell}_{b-1}(A_{b-1})) \right] \label{eqn:2_2}\\ 
    &{\leq}~  \eta N. \label{eqn:2_3}
\end{align}

Eq. (\ref{eqn:2_1}) is because switching is possible only between two consecutive batches. Eq. (\ref{eqn:2_2}) is due to the action selection rule in the algorithm, and Eq. (\ref{eqn:2_3}) is from elementary equality $1-\exp(-x) \leq x, \forall x>0$ and our assumption that each loss is upper bounded by 1.
\end{proof}
\begin{proof}[Proof of Proposition \ref{prop:uniform_alg_upper_bound}]
     Using standard OMD analysis \citep{orabona2019modern}, we have, for any random sequence $\widehat{\ell}_1,\dots,\widehat{\ell}_N$, learning rate $\eta>0$ and one-hot vector $u$, with probability one, we have 
     % \xingyu{for the full information case, do we need this?}
\begin{align}
     \sum_{b=1}^N \left\langle w_b - u, \widehat{\ell}_b \right\rangle &\leq \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K (\widehat{\ell}_b[i])^2 \cdot w_b[i].
\end{align}
%\xingyu{pay attention to subscript.}\duo{fixed}

Taking expectation on both sides, we get
\begin{align}
    \bE\left[ \sum_{t=1}^N \left\langle w_t - u, \widehat{\ell}_t \right\rangle	 \right] &\leq \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K \bE \left[ (\widehat{\ell}_b[i])^2 \cdot w_b[i] \right] \\
    &= \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K \bE \left[ \bE \left[ (\widehat{\ell}_b[i])^2 \cdot w_b[i]| \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right] \\
    &= \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K \bE \left[ \left(\ell_{u_b}[i]\right)^2 \cdot w_b[i] \right] \\
    &\leq \frac{\ln K}{\eta} + \frac{\eta B}{2K}.\label{eqn:generel_OMD_regret_full}
\end{align}
\xingyu{the }
% \duo{$\ell_b$ should be $\ell_{u_b}$, which is always bounded by 1. To be rigorous we should expand the expectation? but the current one is correct right}\xingyu{we can directly use bound for the full info for eq. 49? without local norm?}\duo{Yes, directly batching an existing bound, that's what I did previously and I modified it to this}\xingyu{ok, both are ok. just to check.}

Eq. (\ref{eqn:generel_OMD_regret_full}) is from the boundedness of losses , $\sum_{i=1}^K w_b[i] = 1, \forall b\in\left[N\right]$ and replacing $N$ with $B/K$.

Next we show that $\widehat{\ell}_b$ is indeed an unbiased estimate of the average loss in batch $b$. An important fact to recall here is that $u_b$ is a time slot chosen uniformly at random from the current slot. For any $i \in [K]$, we have

\begin{align}
    \mathbb{E} \left[ \widehat{\ell}_b[i] |\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime}\right] &= \sum_{t = (b-1)\tau+1}^{b\tau} \frac{1}{\tau} \cdot  \ell_{t}[i],\label{eqn:batch_unbiased_estimate_full}
\end{align}
which further indicates that
\begin{align}
\mathbb{E}\left[ \sum_{b=1}^{N} \left\langle w_b - u, \widehat{\ell}_b \right\rangle	 \right] &= \sum_{b=1}^{N} \mathbb{E}\left[ \mathbb{E}\left[ \left\langle w_b - u, \widehat{\ell}_b \right\rangle | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right] \\
&= \sum_{b=1}^{N} \mathbb{E}\left[  \left\langle w_b - u, \mathbb{E}\left[ \widehat{\ell}_b | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right\rangle  \right] \\
&= \sum_{b=1}^{N} \mathbb{E}\left[  \left\langle w_b - u, \frac{ \sum_{i = (b-1)\tau+1}^{b\tau} \ell_{i} }{\tau} \right\rangle  \right] \label{eqn:plug_in_batch_average}\\
&= \frac{1}{\tau} \sum_{b=1}^{N} \sum_{i = (b-1)\tau+1}^{b\tau} \mathbb{E}\left[ \ell_b[A_b] - \ell_b[Y_u]  \right] \\
&= \frac{1}{\tau} \sum_{t=1}^T \mathbb{E}\left[  \ell_t[X_t] - \ell_t[Y_u]  \right],\label{eqn:batch_reduction_full}
\end{align}
where Eq. (\ref{eqn:plug_in_batch_average}) is from Eq. (\ref{eqn:batch_unbiased_estimate_full}) and $Y_u\in[K]$ is the fixed action corresponding to competitor $u$.

Combining Eqs. (\ref{eqn:batch_unbiased_estimate_full}) and (\ref{eqn:batch_reduction_full}), we have
\begin{align}
    \sum_{t=1}^T \mathbb{E}\left[  \ell_t[X_t] - \ell_t[Y_u]\right] &\leq \tau \cdot \left( \frac{\ln K}{\eta} + \frac{\eta B}{2K}\right)\\
    &=\frac{KT\ln K}{\eta B} + \frac{\eta T}{2 },\label{eqn:last_step_regret_full}
\end{align}
where at the last step we replace $\tau$ with $\frac{KT}{B}$.

According to Lemma \ref{lem:SD_switch}, we have
\begin{align}
    \bE \left[\sum_{t=1}^T \bI_{\{X_{t} \neq X_{t-1}\}} \right] \leq \frac{\eta B}{K}.  \label{eqn:switching_cost_upper_bound_full}
\end{align}
Combining Eqs. (\ref{eqn:last_step_regret_full}) and (\ref{eqn:switching_cost_upper_bound_full}), we are finally able to bound the total regret:
\begin{align}
   R_T^{\pi_{\mathrm{full}}} &\leq \frac{KT\ln K}{\eta B} + \frac{\eta T}{2} + \frac{\eta B}{K}\\
    &\leq  \frac{KT\ln K}{\eta B} + \frac{3\eta T}{2}\\
    &=T\sqrt{\frac{6K\ln K}{B}},
\end{align}
where in the second inequality we upper bound $B$ by $KT$ and in the equality we choose $\eta = \sqrt{\frac{2K\ln K}{3B}}$.
\end{proof}

\section{Proof of Proposition \ref{prop:flex upper bound} }\label{app:B<T_upper_bound_proof}
\begin{proof}[Proof of Proposition \ref{prop:flex upper bound}]
    We first consider the case when $B<T$, i.e., $M$ can be any integer from $[K]$.

     Using standard OMD analysis \citep{orabona2019modern}, we have, for any random sequence $\widehat{\ell}_1,\dots,\widehat{\ell}_N$, learning rate $\eta>0$ and one-hot vector $u$, with probability one, we have 
\begin{align}
     \sum_{b=1}^N \left\langle w_b - u, \widehat{\ell}_b \right\rangle &\leq \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K (\widehat{\ell}_b[i])^2 \cdot w_b[i].
\end{align}
Taking expectation on both sides, we get
\begin{align}
    \bE\left[ \sum_{b=1}^N \left\langle w_b - u, \widehat{\ell}_b \right\rangle	 \right] &\leq \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K \bE \left[ (\widehat{\ell}_b[i])^2 \cdot w_b[i] \right] \\
    &= \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K \bE \left[ \bE \left[ (\widehat{\ell}_b[i])^2 \cdot w_b[i]| \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right] \\
    &= \frac{\ln K}{\eta} + \frac{\eta}{2} \sum_{b=1}^N \sum_{i=1}^K \bE \left[ \left(\frac{\ell_{u_b}[i]}{M/K}\right)^2 \cdot w_b[i] \cdot \frac{M}{K} + 0 \cdot (1-\frac{M}{K}) \right] \\
    &\leq \frac{\ln K}{\eta} + \frac{\eta  KB}{2M^2},\label{eqn:generel_OMD_regret_generel_full}
\end{align}
where is from the boundedness of losses , $\sum_{i=1}^K w_t[i] = 1, \forall t\in\left[T\right]$ and replacing $N$ with $B/M$.

Next we show that $\widehat{\ell}_b$ is indeed an unbiased estimate of the average loss in batch $b$. For any $i \in [K]$, we have

\begin{align}
    \mathbb{E} \left[ \widehat{\ell}_b[i] |\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime}\right] &= (1-\frac{M}{K}) \cdot 0 + \frac{M}{K} \cdot \sum_{t = (b-1)\tau+1}^{b\tau} \frac{1}{\tau} \cdot  \frac{\ell_{t}[i]}{M/K} \\
    &= \frac{ \sum_{t = (b-1)\tau+1}^{b\tau} \ell_{t}[i] }{\tau},\label{eqn:batch_unbiased_estimate_general_full}
\end{align}
which further indicates that
\begin{align}
\mathbb{E}\left[ \sum_{b=1}^{N} \left\langle w_b - u, \widehat{\ell}_b \right\rangle	 \right] &= \sum_{b=1}^{N} \mathbb{E}\left[ \mathbb{E}\left[ \left\langle w_b - u, \widehat{\ell}_b \right\rangle | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right] \\
&= \sum_{b=1}^{N} \mathbb{E}\left[  \left\langle w_b - u, \mathbb{E}\left[ \widehat{\ell}_b | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right\rangle  \right] \\
&= \sum_{b=1}^{N} \mathbb{E}\left[  \left\langle w_b - u, \frac{ \sum_{i = (b-1)\tau+1}^{b\tau} \ell_{i} }{\tau} \right\rangle  \right] \label{eqn:5_3}\\
&= \frac{1}{\tau} \sum_{b=1}^{N} \sum_{i = (b-1)\tau+1}^{b\tau} \mathbb{E}\left[ \ell_b[A_b] - \ell_b[Y_u]  \right] \\
&= \frac{1}{\tau} \sum_{t=1}^T \mathbb{E}\left[  \ell_t[X_t] - \ell_t[Y_u] \right],\label{eqn:batch_reduction_general_full}
\end{align}
where Eq. (\ref{eqn:5_3}) is from Eq. (\ref{eqn:batch_unbiased_estimate_general_full}) and $Y_u$ is the fixed action corresponding to competitor $u$.

Eqs. (\ref{eqn:generel_OMD_regret_generel_full}) and (\ref{eqn:batch_reduction_general_full}) indicate that
\begin{align}
    \sum_{t=1}^T \mathbb{E}\left[  \ell_t[X_t] - \ell_t[Y_u]\right] &\leq \tau\cdot\left( \frac{\ln K}{\eta} + \frac{\eta  KB}{2M^2}\right)\\
    &=\frac{MT\ln K}{\eta B} + \frac{\eta T K}{2M },\label{eqn:last_step_regret_general_full}
\end{align}
where in last step we replace $\tau$ with $\frac{MT}{B}$.

According to Lemma \ref{lem:SD_switch}, we have
\begin{align}
    \bE \left[\sum_{t=1}^T \bI_{\{X_{t} \neq X_{t-1}\}} \right] \leq \eta N \frac{ K}{M}=\frac{\eta BK}{M^2}.  \label{eqn:switching_cost_upper_bound_general_full}
\end{align}
Combining Eqs. (\ref{eqn:last_step_regret_general_full}) and (\ref{eqn:switching_cost_upper_bound_general_full}), we are finally able to bound the total regret:
\begin{align}
   R_T^{\pi_{\mathrm{flex}}} &\leq \frac{MT\ln K}{\eta B} + \frac{\eta T K}{2M} + \frac{\eta BK}{M^2}\\
    &\leq  \frac{MT\ln K}{\eta B} + \frac{3\eta KT}{2M}\\
    &=T\sqrt{\frac{6K\ln K}{B}},
\end{align}
where in the second inequality we upper bound $B$ by $MT$ (recall that now $B<T$ and $M\geq 1$) and in the equality we choose $\eta = M\sqrt{\frac{2\ln K}{3BK}}$.

The proof for $B\geq T$ is exactly the same, except for the (implicit) fact that we need batch size $\tau$ to be well-defined, i.e., $\tau\geq 1$. That's why in this case $M$ is less flexible: now $M$ needs to be sufficiently large to fully exploit the total budget.
\end{proof}

\section{Proof of Proposition \ref{prop:bandit_upper_bound}}\label{app:bandit_upper_bound_proof}
\begin{proof}[Proof of Proposition \ref{prop:bandit_upper_bound}]
 Using standard OMD analysis \citep{orabona2019modern}, we have, for any random sequence $\widehat{\ell}_1,\dots,\widehat{\ell}_N$, learning rate $\eta>0$ and one-hot vector $u$, with probability one, we have
\begin{equation}
 \sum_{b=1}^{N} \left\langle w_b - u, \widehat{\ell}_b \right\rangle  \leq \frac{\ln K}{\eta} + \frac{\eta}{2}\sum_{b=1}^{N} \sum_{i=1}^K (\widehat{\ell}_b[i])^2 w_b[i]. \label{eqn:5_1}
\end{equation}
Taking expectation on both sides, we have
\begin{align}
\bE\left[\sum_{b=1}^{N} \left\langle w_b - u, \widehat{\ell}_b \right\rangle \right] &\leq \frac{\ln K}{\eta} + \frac{\eta}{2}\sum_{b=1}^{N} \bE\left[\sum_{i=1}^K (\widehat{\ell}_b[i])^2 w_b[i]\right]\\
&= \frac{\ln K}{\eta} + \frac{\eta}{2}\sum_{b=1}^{N} \ex{\ex{\sum_{i=1}^K (\widehat{\ell}_b[i])^2 w_b[i]\bigg|\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime}}}\\
&= \frac{\ln K}{\eta} + \frac{\eta}{2}\sum_{b=1}^{N}\ex{ \sum_{i=1}^K w_b[i] \cdot \frac{1}{\tau} \cdot \sum_{t = (b-1)\tau+1}^{b\tau} \frac{(\ell_t[i])^2}{(w_b[i])^2} \cdot w_b[i]}\\
&\leq \frac{\ln K}{\eta} + \frac{\eta}{2}NK\\
&= \sqrt{2NK\ln K},\label{eqn:5_5}
\end{align}
where the last inequality follows the assumption that all losses are bounded by one and $\sum_{i=1}^K w_b[i] = 1, \forall b \in [N]$, and the last equality is obtained by selecting $\eta = \sqrt{\frac{2\ln K}{NK}}$.
%\duo{I still think that there shouldn't be an expectation at the LHS above, since here we fix the loss sequence, i.e., all $u_b$'s, in this case, there's no random variable at LHS, am I wrong?} \xingyu{I think Eq. 23 is very confusing to me (why? since in standard result of EXP3, we do not have $w_b$ on LHS, which is a probability vector. Rather, we only has the actual pulled action. Then, we need expectation). A suggestion is to directly use OMD with estimations to prove regret of Algorithm 1 as discussed above (nearly the same as in the non-batch case .), i.e., follow Thm 12.5 in my note \url{https://drive.google.com/file/d/1k-yWao8HcYjbWYdpcMb-SzQvRbiNrAd1/view}}\duo{sure. I'll complete the proof, but what I mean by eqn.23 (removing the expectation and before selecting $\eta$) is the eqn 12.16 in your note, if that helps to clarify}
%\xingyu{yes, it is equal to 12.16. Then, you just need to bound the local norms, then done.}
%\duo{I see, then seemingly we are on the same page :)}\xingyu{yes:) the main point is that it seems to me we cannot directly use reduction to EXP3 as in~\cite{Dekel2012OnlineBL}. Rather, we have to start from 12.16 to re-prove it.}

Next we need to check if $\widehat{\ell}_b$ is indeed an unbiased estimate of the average loss in batch $b$. Notice that $u_b$ is independent of the choice of action, hence we have for any $i \in [K]$,
%\duo{here there're two layers of randomness, one is selecting the action and the other is choosing the time slot for feedback. They are independent.}
\begin{align}
    \mathbb{E} \left[ \widehat{\ell}_b[j] |\widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime}\right] &= (1-W_b[j]) \cdot 0 + \sum_{t = (b-1)\tau+1}^{b\tau} \frac{1}{\tau} \cdot W_b[i] \cdot \frac{\ell_{t}[i]}{W_b[i]} \\
    &= \frac{ \sum_{t = (b-1)\tau+1}^{b\tau} \ell_{t}[i] }{\tau}. \label{eqn:5_2}
\end{align}

Combining Eqs. (\ref{eqn:5_5}) and (\ref{eqn:5_2}), we have
\begin{align}
\mathbb{E}\left[ \sum_{b=1}^{N} \left\langle w_b - u, \widehat{\ell}_b \right\rangle	 \right] &= \sum_{b=1}^{N} \mathbb{E}\left[ \mathbb{E}\left[ \left\langle w_b - u, \widehat{\ell}_b \right\rangle | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right] \\
&= \sum_{b=1}^{N} \mathbb{E}\left[  \left\langle w_b - u, \mathbb{E}\left[ \widehat{\ell}_b | \widehat{\ell}_1 = \ell_1^{\prime}, \dots, \widehat{\ell}_{b-1} = \ell_{b-1}^{\prime} \right] \right\rangle  \right] \\
&= \sum_{b=1}^{N} \mathbb{E}\left[  \left\langle w_b - u, \frac{ \sum_{i = (b-1)\tau+1}^{b\tau} \ell_{i} }{\tau} \right\rangle  \right] \label{eqn:5__3}\\
&= \frac{1}{\tau} \sum_{b=1}^{N} \sum_{i = (b-1)\tau+1}^{b\tau} \mathbb{E}\left[ \ell_i[A_b] - \ell_i(Y_u)  \right] \\
&= \frac{1}{\tau} \sum_{t=1}^T \mathbb{E}\left[  \ell_t[X_t] - \ell_t[Y_u]  \right] \\
&\leq \sqrt{2N K\ln K },
\end{align}
where Eq. (\ref{eqn:5__3}) is from Eq. (\ref{eqn:5_2}) and $Y_u$ is the fixed action corresponding to competitor $u$. Now we can see that:
\begin{align}
\sum_{t=1}^T \mathbb{E}\left[  \ell_t[X_t] - \ell_t[Y_u]  \right] &\leq \tau \sqrt{2N K\ln K} \\
&= \frac{T}{B} \cdot \sqrt{2 B K \ln K} \\
&= O\left( T \sqrt{\frac{K\ln K}{B}}\right). \label{eqn:5_4}
\end{align}

When $B = O(\PTP)$, we have $\sum_{t=1}^T \mathbb{I}_{\{X_{t} \neq X_{t-1}\}} \leq B = O( T \sqrt{\frac{K\ln K}{B}})$. Combining it with Eq. (\ref{eqn:5_4}), finally we obtain our desired result.
\end{proof}





==> notes.tex <==
% Checklist
% \begin{itemize}

% \item rewrite related work (done)
% \item rewrite Remark 7 (Bo; done)
% \item check the first two paragraphs of Section 4 (Bo; done - added back (Q3))
% \item refer back to Table 1 in Section 4 (Bo; done - see Remark 8)
% \item carefully read appendix (Xingyu first, then Bo)
% \item revisit abstract and conclusion (Xingyu)
% \item modify proof of Proposition 1 in a separate file (Duo)(Done, not in a separate file but I have backup)
% \item check whether all remarks and footnotes are necessary (Duo)(Done, I feel like every remark/footnote is useful...)\bo{I removed the original footnote 2 (about ignoring $K$) and simplified the others.}
% \item revisit the contribution bullets

% \end{itemize}

%I think space is no longer an issue now. It remains to revise the conclusion and contribution bullets. Then, we should focus on the appendix.

%\bo{Duo, please change two $B_{\mathrm{extra}}$'s to $\Bex$ in Fig.~1(a). Double check other places as well.}\duo{Done}

%\bo{Duo, if you have some time later, you may want to do a quick search and see if you have missed any relevant work, especially more recent ones}\duo{this 2018 paper \url{https://alinlab.kaist.ac.kr/resource/Multi_armed_Bandit_with_Additional_Observations.pdf} studies stochastic and adversarial bandits with add.tional feedback without switching costs, and the learner can choose which arms to observe.}\bo{then you need to cite and discuss this paper as well, focusing the discussion on the adversarial setting. What is the main message/conbribution of this paper?}\duo{they achieve tight bound w.r.t. $K$, $T$ and $M$ (no additional poly-log factors), at each round, the learner observes $M-1$ additional actions ($M=1$ is bandit, $K-1$ is full) at her choice. one contribution is their alg. design ``H-INF''.}
\duo{in terms of switching costs, I don't find any new work}\bo{also, can their application be used for your another motivating example for feedback budget as well?}

%\duo{remains to check the first bullet of contribution, the table and the conclusion.}\duo{and proof}

%\bo{remember to change tilde notation for the budget throughout the paper after you are done with the new proof.}\duo{I remember but I planned to do that after you two go trough the proof and makes sure it's no problem}

%\bo{I think one important message is currently missing. What makes the type important? Duo said in the setting without switching costs under a total budget, bandit feedback can also achieve the optimal regret (which needs a simple proof using batched EXP3), i.e., the type does not really matter. With this, we should further explain that the impact of feedback type comes from switching costs. Potentially, we should add one more column to Table 1 for the setting without switching costs to make a contrast. We can come back to this later though.}
%\duo{the proof is exactly our last equation in the appendix. regret (without switching costs) holds for any $B\leq T$, but only when $B$ is small, the switching costs is a lower order term, that's it. }

%\bo{we need to use/explain this new Table 1 well wherever we refer to it}
%\duo{we refer to it in the 3rd contribution and the end of sec 4.}\duo{added new message at the end of sec 4}

%\bo{the motivating example is not convincing to me}

%\bo{I revised the contribution bullets following the abstract.}

\duo{todo: remove lots of tilde in the main body}\bo{make sure to double check the entire paper to ensure consistency. Also, double check the correctness of the lower bound proof after this modification}

\bo{I am comfortable with the paper except for the motivating examples. And I haven't carefully read the proofs yet.}

\bo{ICML used to ask authors to choose topics in the submission site. I do not see it this time. Did I miss anything? In this case, make sure that you provide the most relevant key works. For example, no need to include ``online convex optimization''}\duo{Ok, i'll ask Dr. Zhou to double check}\duo{they use matching alg. for reviewer assignment (according to key words?)}

%\bo{In openreview, let's try to add the following: TLDR "Too Long; Didn't Read": a short sentence describing your paper. Xingyu, can you add one short sentence?}

\bo{you can add the shade to the big L-shape area in Table~1 if you have time; also move the bound down a little bit so that it sits in the middle, vertically, but these are less important}


==> sec4.tex <==
\section{Bandit Learning with Switching Costs under Extra Observation Budget}\label{sec:extra}
%\duo{have changed the thm. statement into minimax, and mentioned the upper bound at the last line of sec 4. the title/division of subsec 4.3 4.4 may be weird}

Observing the gap in the optimal regret bound under bandit and full-information feedback ($\wtTheta(T^{2/3})$ vs. $\Theta(\sqrt{T})$),\footnote{In the rest of the paper, we will focus on the dependency on $T$ and may omit terms involving $K$ whenever the context is clear.}
%\bo{add a footnote to explain that we will focus on the dependency on $T$ throughout the rest of the paper}\duo{done}, 
it is natural to ask: 
\emph{How much can one improve upon the $\wtTheta(T^{2/3})$ regret if the learner is allowed to make some extra observations in addition to the typical bandit feedback?} 
%In particular, if the learner can freely make no more than $\Bex$ extra observations throughout the game, what would be the optimal regret with respect to both $T$ and $\Bex$?

Motivated by this question, we consider the setting of bandit learning with switching costs under an \emph{extra} observation budget. Under the learning protocol specified in \secref{problem setup}, in addition to the typical bandit feedback, the learner is allowed to freely use at most $\Bex$ extra observations of the loss of other action(s) throughout the game, where $\Bex$ is an integer in $[0, (K-1)T]$. At the two endpoints of $0$ and $(K-1)T$, this new setting recovers the bandit and full-information cases, respectively. In this section, by slightly abusing the notation, we use $\Pi$ to denote the set of all learning algorithms using typical bandit feedback plus $\Bex$ extra observations, and 
we are interested in the minimax regret $R^*_T$ for $\Bex \in [0, (K-1)T]$.
%\bo{you used this term, but never rigorously defined it}\duo{done. defined in eq. \ref{eqn:minimax_reg_def}}
% for general $\Bex$ in this range. Hence in this setting, $\Pi$ becomes the set of all learning algorithms relying on bandit feedback plus $\Bex$ extra observation.

\subsection{Minimax Regret}
We first present our main result of the minimax regret $R_T^*$ in this setting, which is formally stated in \thmref{bandit_extra_minimax}.
%To show this lower bound, we adopt the instance construction from \citet{shi2022power}, which is further a modification based on the multi-scale random walk proposed by \citet{dekel2014bandits}, with our refined analysis. \bo{The current way of writing may get the reader distracted to think about the difference between your work and \citet{shi2022power}. We should just say that our main idea is based on the multi-scale random walk here and mention \citet{shi2022power} later and explain the difference}\duo{can I keep the first sentence only? everything regarding the instance construction will be addressed in proof sketch}

%\bo{Use different counters for lemmas, theorems, remarks, etc.}\duo{done}
\begin{theorem}\label{thm:bandit_extra_minimax}
    In the setting of bandit learning with switching costs under an extra observation budget $\Bex \in [0, (K-1)T]$, the minimax regret is given by
    \begin{equation*}
        R_T^*=\left\{
        \begin{aligned}
        &\wtTheta(\PTP), & ~\text{if}~\Bex=\wtO(\PTP), \\
        &\wtTheta(T\sqrt{K/\Bex}), & ~\text{if}~\Bex=\wtOmega(\PTP).
        \end{aligned}
        \right.
    \end{equation*}
\end{theorem}

%\bo{Since you focus on the minimax optimal regret $R_T^*$, I think you should state Theorem~1 based on a lower bound on the minimax optimal regret $R_T^*$. Then, you can probably use a big bracket with two cases, and no need to mention any learning algorithm and the existence of a loss sequence here in the statement (but only in the proof and/or proof sketch). Also check how other papers deal with this.}

%\bo{I think we can simply use $R^*_T$. In Section 5, we can say that by slightly abusing the notation, we also use $\Pi$ and $R^*_T$}\duo{for sure we can do that, but what's wrong this the current one which avoids further ambiguity?}\bo{I think this notation is unnecessarily complicated}

%\bo{Can we use the big bracket notation for two cases?}\duo{done}

%\bo{Similar comment for the upper bound.}\duo{I don't think we should mention minimax bound in the theorem statement of upper bound. However we can/should interpret it after the upper bound theorem}\bo{Why not? You can have a similar statement. In the proof sketch and proof, you can say that there exists an algorithm...}\duo{but we also need to introduce different algorithms}
%\bo{That is fine - it does not impact the theorem statement} \duo{we have theorem \ref{thm:general_upper_bound}, which is sufficient since it fully characterizes the optimal regret. after that we can focus on introducing the algorithm}
%\bo{That's what I meant by upper bound. For the propositions, of course, you need to introduce algorithms.}

%\bo{make this paragraph a remark?}\duo{done}

\begin{remark}
This minimax regret exhibits an interesting phase-transition phenomenon (cf. Fig.~\ref{fig:case 1}): when the number of extra observations is relatively small (i.e., $\Bex = \wtO(\PTP)$), these extra observations are insufficient to help improve the regret no matter how they are used, and the regret remains $\Theta(T^{2/3})$; however, when sufficiently many extra observations are available (i.e., $\Bex = \wtOmega(\PTP)$), the regret decreases as the number of extra observations increases.
\end{remark}

To prove Theorem~\ref{thm:bandit_extra_minimax}, we need to show a fundamental lower bound and provide algorithms that can achieve this lower bound. Next, we present a lower bound of the minimax regret. The result is stated in the following proposition.

\begin{proposition}\label{prop:bandit_extra_lower_bound}
     In the setting of bandit learning with switching costs under an extra observation budget $\Bex \in [0, (K-1)T]$, the minimax regret has the following lower bound:
    \begin{equation*}
        R_T^*=\left\{
        \begin{aligned}
        &\wtOmega(\PTP), & ~\text{if}~\Bex=\wtO(\PTP), \\
        &\wtOmega(T\sqrt{K/\Bex}), & ~\text{if}~\Bex=\wtOmega(\PTP).
        \end{aligned}
        \right.
    \end{equation*}
\end{proposition}

\subsection{Proof Sketch of the Lower Bound}
In this subsection, we will walk through the main steps of the lower bound analysis with necessary explanations. After that, we will further show that some observations from this lower bound analysis indeed motivate our algorithm design
so that we can match this lower bound, which will be discussed later in this paper. The detailed lower bound proof is in Appendix~\ref{app:extra_lower_bound_proof}. 
In the following, we explain the main idea of it along with a proof sketch and provide useful insights into the interesting phase-transition phenomenon. 

    To prove this lower bound, it suffices to show that for any learning algorithm $\pi$ that can use a total of $\Bex$ extra observations in addition to bandit feedback, there exists a loss sequence $\ell_{1:T}$ (which may depend on both $\pi$ and $\Bex$) such that when $\Bex = \wtO(\PTP)$, we have $\ex{R_T^{\pi}(\ell_{1:T})} =  \wtOmega(\PTP)$; and when $\Bex = \wtOmega(\PTP)$, we have $\ex{R_T^{\pi}(\ell_{1:T})} =  \wtOmega( T\sqrt{K/\Bex})$.\duo{how about making this statement as proposition 1? In this case we can avoid repeat theorem 1 twice (only Theta is replaced by Omega)}
    %\bo{Is the construction the same in two cases or not?}\duo{no. e.g., the choice of $\epsilon$ is different.}
    
    We first give an overview of the construction of such loss sequences and the main ideas behind that.

    Generally speaking, the difficulty of bandit problems lies in the \emph{exploitation-exploration} tradeoff.
    %\bo{be consistent throughout the paper; I'd prefer to use ``tradeoff'' as it is now adopted as a single word; similar for nontrivial, nonnegative, etc.; check dictionary}
    Since the environment is unknown, on the one hand, the learner may want to pull the empirically good actions in order to enjoy low instantaneous loss (i.e., exploitation); on the other hand, she may also want to pull other actions and gain useful information to distinguish the optimal action (i.e., the best fixed action) and suboptimal actions (i.e., exploration).
    %gain more distinguishability on the identity of the underlying optimal action (i.e., exploration).

    In the presence of switching costs,
    %\duo{how about deleting: (one intuitive way to construct hard instances is to \duo{construct a relationship between} switches and exploration. \bo{``connect'' is unclear} In particular,)}
    \citet{dekel2014bandits} proposes loss sequences based on a multi-scale random walk such that useful information (i.e., distinguishability of the optimal action and suboptimal actions) is obtained \emph{only when the learner switches actions}, which, however, incurs switching costs. Using carefully constructed instances, they show that switching costs increase the intrinsic difficulty of bandit learning and result in a lower bound of $\wtOmega(T^{2/3})$. 

    However, the hard instances in \citet{dekel2014bandits} work for \emph{pure bandit feedback} only. That is, if the learner can obtain full-information feedback in \emph{any} one of the $T$ rounds, she will immediately identify the optimal action and suffer no regret in the rest of the game. The reason is that the optimal action has uniquely lowest loss at \emph{all} $T$ rounds.

    To make it still hard to learn even when the learner has some additional feedback, we will borrow an idea used in \citet{shi2022power} (for a different problem) to modify the original hard instance: at each round, an additional layer of action-dependent noise is added to the loss of each action. As a result, the optimal action no longer has the lowest loss at all rounds and therefore cannot be easily identified even when the learner can make additional observations beyond the typical bandit feedback. 

    In the rest of this proof sketch, we present three key steps of the proof and provide high-level explanations. 
    %\bo{what are the illustrations here?}\duo{by ``illustrations'' I meant ``explanations''}\bo{how about ``provide high-level explanations''}\duo{done}
    
    % In the rest of this proof sketch, we follow the organization of Appendix G.3 from \citet{altschuler2018online} to show key steps and deliver some illustrations.
    
    \paragraph{Step 1: Establishing the relationship between regret and unclipped regret.} 
    %\bo{Here, it is unclear what kind of random walk you refer to and what the truncated version is used for. You need to explain it clearly.}
    Let $\ell_{1:T}^{\mathrm{unclipped}}$ be the loss sequence generated by the random walk from the Algorithm 1 in \citet{shi2022power} (which is not necessarily bounded in $[0,1]$) and $\ell_{1:T}$ be its truncation to $[0,1]$\footnote{Specifically, $\ell_t[k] =  \min_{x\in[0,1]}\left|x-\ell_t^{\mathrm{unclipped}}[k]\right|, \forall k\in[K], t\in[T]$, namely, the number nearest to $\ell_t^{\mathrm{unclipped}}[k]$ in $[0,1]$.}. Recall that for any given learning algorithm $\pi$, $\ex{R^{\pi}_T(\ell_{1:T}^{\mathrm{unclipped}})}$ and $\ex{R^{\pi}_T(\ell_{1:T})}$ are the expected regret over these two sequences, respectively. For notational ease, we use $\ex{R_T^{\mathrm{unclipped}}}$ and $\ex{R_T}$ to denote them respectively in the rest of this section.
    %Let $\ex{R_T^{\mathrm{unclipped}}}$ and $\ex{R_T}$ be the expected regret (for any given learning algorithm) over these two sequences, respectively, where the randomness is due to loss generation. 
    Our ultimate goal is to obtain a lower bound on $\ex{R_T}$ (i.e., regret over the truncated loss), which, however, is hard to analyze directly due to the truncation. To handle this, we establish the relationship between $R_T$ and $R_T^{\mathrm{unclipped}}$ by showing that for any sufficiently large $T$, the following holds:
    \begin{align}\label{eqn:unclipped_bounds_clipped}
        \ex{R_T} \geq \ex{R_T^{\mathrm{unclipped}}} - \frac{\epsilon T}{6},
    \end{align}
    where $\epsilon>0$ is the per-round loss gap between the optimal action and the suboptimal actions. We will determine the value of $\epsilon$ later. \eqnref{unclipped_bounds_clipped} implies that a lower bound on $\ex{R_T^{\mathrm{unclipped}}}$ also leads to a lower bound on $\ex{R_T}$. Therefore, in the rest of the analysis, it suffices to focus on the unclipped loss and lower bound $\ex{R_T^{\mathrm{unclipped}}}$.

\paragraph{Step 2: Lower bounding $\ex{R_T^{\mathrm{unclipped}}}$ in terms of the number of switches and extra observations.}
%\xingyu{upper bound the distinguishability, hence lowering bound the regret?}\duo{yes, that's the precise expression and hard to formulate using just one sentence. Can I just ignore the distinguishability like the current one? since this will be elaborated on later in the proof sketch.}\xingyu{yes, this is fine}

Through a careful information-theoretic analysis, we can obtain the following (informal) lower bound on $\ex{R_T^{\mathrm{unclipped}}}$:
\begin{align}
   \ex{R_T^{\mathrm{unclipped}}} &\geq\nonumber \\
   \underbrace{\!\frac{\epsilon T}{2}}_{\mathbf{A.1}}&\!-\!\underbrace{C \frac{ \epsilon^2 T }{\sqrt{K}} \left( \sqrt{ N^s} \!+\!  \sqrt{ \Bex}\right)}_{\mathbf{A.2}} \!+\! \underbrace{N^s}_{\mathbf{A.3}}\label{eqn:extra_lower_bound_before_minimize},
\end{align}
where $C>0$ contains some universal constants and polylogarithmic terms of $T$, and $N^s$
%\bo{use $N^s$ instead? Actually, why not simply $N^s$?}\duo{because $N^s$ has been used in theappendix for different meaning.} 
denotes the total number of switches that have occurred. 
%\bo{Is it possible that you use $N^s$ here and use $\bar{N}^s$ where you currently use $N^s$?}\duo{done}\bo{Make sure to double check when you simply find and replace. It still has the bar in $\bar{N}_*^s$}\duo{I have iterated every ``bar'' command}
%Here, we choose $\sigma=\Theta(1/\log{T})$, which is contained in $C_1$. \bo{There is no $\sigma$. Delete this sentence?}\duo{Yes. I forgot about it}

%We now explain each term on the right-hand side (RHS) of \eqnref{extra_lower_bound_before_minimize}. $\mathbf{A.1}$ %\bo{remove the word ``Term'' in the equations?}\duo{done}is the regret that the learner will suffer without any distinguishability \bo{you use distinguishability a lot here; make sure you explain this clearly the first time you use this term}\duo{I explain it in the newly-added paragraph which introduces the ex-ex dilemma}, namely, $\Theta(\epsilon T)$ \bo{why is there $1/2$ in A.1?}. $\mathbf{A.2}$ corresponds to  how much information the learner collects that is useful for distinguishing the optimal 
%\bo{use ``optimal'' throughout the paper?}\duo{I can do that but it's a little weird to say ``optimal fixed action''. Ppl normally say ``optimal fixed'' }\duo{done} action from suboptimal actions: better distinguishability leads to a larger $\mathbf{A.2}$, which further leads to a smaller regret lower bound. $\mathbf{A.3}$ is simply the switching costs incurred.

We now explain each term in the above lower bound.
%on the right-hand side (RHS) of \eqnref{extra_lower_bound_before_minimize} to characterize how the lower bound is established. 
Term~$\mathbf{A.1}$ reflects that without any distinguishability, the learner may be stuck with a suboptimal action throughout the game, thus suffering $\Theta(\epsilon T)$ regret. Term~$\mathbf{A.2}$ roughly reveals how much information collected by the learner is useful for gaining distinguishability and thus reducing the regret: better distinguishability leads to a larger $\mathbf{A.2}$, which further leads to a lower regret. 
Term~$\mathbf{A.3}$ is simply the switching costs incurred.

\paragraph{Step 3: Choosing $\epsilon$ according to the value of $\Bex$.}
Note that the lower bound in \eqnref{extra_lower_bound_before_minimize} is a quadratic function of $\sqrt{N^s}$. By finding the minimizer of this quadratic function, we can further obtain the following lower bound:
\begin{align}
    \ex{R_T^{\mathrm{unclipped}}} \geq
   \underbrace{\frac{\epsilon T}{2}}_{\mathbf{B.1}}-~\underbrace{\frac{C^2}{4}\cdot \frac{ \epsilon^4 T^2 }{K}}_{\mathbf{B.2}} - \underbrace{C\frac{\epsilon^2 T\sqrt{\Bex}}{\sqrt{K}}}_{\mathbf{B.3}}.
   \label{eqn:lower_bound_after_minimize}    
\end{align}
 %where $C_2$ and $C_3$ \bo{shouldn't we simply have $C_3=C_1$ and $C_2=C_1^2$? If so, just use $C$ instead of $C_1$}\duo{yes, fixed}\xingyu{no $C_2$ $C_3$ now} contain some universal constants and logarithmic terms of $T$.
 It now remains to choose a proper value of $\epsilon$. 
 %\bo{Does this imply the construction is the same for these two cases?}\duo{in some sense yes. only the choice of $\epsilon$ is different}
 By considering two different cases (i.e., $\Bex=\wtOmega(\PTP)$ and $\Bex=\wtO(\PTP)$) and choosing $\epsilon$ accordingly,
 %\bo{it would be easier for the reader to see if you can explain how to choose $\epsilon$ and give the choice of $\epsilon$. otherwise, it would also be harder to follow the insights discussed below}\duo{the following paragraphs explain how $\epsilon$ is chosen and leads to different lower bounds. Do we need to state here again?}
 we show that one of terms $\mathbf{B.2}$ and $\mathbf{B.3}$ will dominate the other. Then, we can obtain the desired lower bound by combining these two cases, which ends this proof sketch.
%\duo{added one remark}

\begin{remark}\label{remark:purdue}
    While we use the same instance construction method in \citet{shi2022power}, the problem they study is very different from ours. In particular, their learning protocol as well as the definition of switching costs are different. We refer the reader to Appendix \ref{app:purdue_difference} for a further discussion.%\xingyu{it is not easy for understanding. You can just say that their problem is different in terms of problem setup and regret definition. Then, refer to Appendix for further discussion. No need to give details here}\duo{done}
\end{remark}

\subsection{Insights from Lower Bound}
Next, we give some useful insights and observations that can be obtained from the above proof sketch, in particular, \eqnref{extra_lower_bound_before_minimize}, which provides a \emph{unified} view of the lower bound in online learning with bandit feedback and flexible extra observations within a total budget.

As a warm-up, we begin with the standard bandit case (i.e., $\Bex = 0$), which has been extensively studied~\cite{dekel2014bandits}. Recall that under the current instance construction, bandit feedback provides useful information \emph{only} when the learner switches actions. From \eqnref{extra_lower_bound_before_minimize}, one can observe that there is a tradeoff between exploration and switching costs: in order to better explore and enjoy a lower regret, the learner has to switch frequently (i.e., a larger $N^s$) so as to gain more information (i.e., a larger $\mathbf{A.2}$). However, since the learner has to pay one unit of switching cost for each switch (contributing to $\mathbf{A.3}$), she should not switch too much. For example, if the learner switches $T$ times, the regret would already be $\Omega(T)$ purely due to the switching costs. Therefore, to strike the balance between the two, the best the learner can do is to switch $N_*^s = \wtTheta(\PTP)$ (otherwise the regret can only be worse as $N_*^s$ is the minimizer of the RHS of \eqnref{extra_lower_bound_before_minimize}). Finally, choosing $\epsilon$ to be $\wtTheta(K^{1/3}T^{-1/3})$ in \eqnref{lower_bound_after_minimize} yields the lower bound of $\wtOmega(\PTP)$ for the bandit case. 
%Finally, choosing $\epsilon$ to be $\wtTheta(K^{1/3}T^{-1/3})$ in \eqnref{lower_bound_after_minimize} yields the lower bound of $\wtOmega(\PTP)$ for the bandit case.

%Now, we consider the first case: $\Bex=\wtO(\PTP)$. After going through how we obtain the lower bound of $\wtOmega(\PTP)$ for the bandit case, it might be easier to see why $\wtO(\PTP)$ extra observations are not sufficient to improve the minimax regret: let $N^s$ and $\epsilon$ still take the same value as in the bandit case (i.e., $\wtTheta(K^{1/3}T^{2/3})$ and $\wtTheta(K^{1/3}T^{-1/3})$, respectively); although $\mathbf{B.3}$ in \eqnref{lower_bound_after_minimize} now becomes positive instead of zero (as in the bandit case), it is still dominated by $\mathbf{B.2}$, which results in the same regret of $\wtOmega(\PTP)$ as in the bandit case. In other words, although the learner can now make some extra observations that help obtain additional information, the gain is too small to improve the regret order-wise.

%\duo{rewrite $\uparrow$ (actually I just swap the first and second half):}
Now, we consider the first case: $\Bex=\wtO(\PTP)$. In this case, one might hope to obtain a smaller regret with the help of additional feedback.
%However, after going through how we obtain the regret lower bound of $\wtOmega(\PTP)$ for the bandit case, it might be easier to see why $\wtO(\PTP)$ extra observations are insufficient to improve the minimax regret: intuitively, although the learner can now make some extra observations that help obtain additional information, the gain is too small to improve the regret order-wise.
However, we'll show that unfortunately, the gain from those additional observations is too small to improve the regret order-wise, and hence the previous $\wtOmega(\PTP)$ bound remains. To see this, let $N^s$ and $\epsilon$ still take the same value as in the bandit case (i.e., $N^s=\wtTheta(K^{1/3}T^{2/3})$ and $\epsilon=\wtTheta(K^{1/3}T^{-1/3})$);
%\bo{why choose the same $N^s$ and $\epsilon$? People may ask: would other choices be helpful?}\duo{because with additional observation, the (tight) lower bound can only be smaller compared to the bandit case. However this is not true due to what we show. I've adjusted this paragraph accordingly to highlight this.}
although $\mathbf{B.3}$ in \eqnref{lower_bound_after_minimize} now becomes positive instead of zero (as in the bandit case), it is still dominated by $\mathbf{B.2}$, which results in the same regret of $\wtOmega(\PTP)$ as in the bandit case.

%\bo{this part is unclear and needs to be rewritten}\duo{rewritten below} Finally, we consider the second case: $\Bex = \wtOmega(\PTP)$. In this case, extra observations are sufficient in the sense that the regret  help improve the regret to $\wtOmega(T\sqrt{K/\Bex})$. Consequently, by a different choice of $\epsilon = \wtTheta(\sqrt{K/\Bex})$, now $\mathbf{B.3}$ is dominating $\mathbf{B.2}$ and we arrive at our desired result. That is to say, now the improved bound comes from better exploration (which corresponds to $\mathbf{A.2}$) due to a sufficient amount of extra observations (which however will not incur extra switching costs) so that the learner now does not have to necessarily switch $\wtTheta(T^{2/3})$ times in order to explore well.

%\duo{rewrite the $\uparrow$ paragraph}
Next, we consider the second case: $\Bex = \wtOmega(\PTP)$. In contrast to the previous case, due to the relatively large budget, the distinguishability provided by those additional observations (which do not contribute to switching costs) is no longer negligible, which leads to a smaller lower bound. In particular, by choosing $\epsilon = \wtTheta(\sqrt{K/\Bex})$, we will make $\mathbf{B.3}$ dominate $\mathbf{B.2}$ and obtain the desired lower bound. In other words, one can reduce the regret through better exploration enabled by sufficient extra observations that do not incur switching costs.
%\bo{use the integrated tool Grammarly in overleaf to help you spot and fix such minor editorial issues (typos, misspellings, grammatical mistakes, etc.); make sure to think about the suggestions provided by the tool though}\duo{sure, typically I'll try to figure it out whenever I see an error suggested.}
%\xingyu{you might need to write the previous paragraph (when extra obs is small) like this paragraph. That is, first give the intuition and then give the math.} \duo{done}
%\paragraph{Connections to upper bound and algorithm design.} 

\subsection{Insights into Algorithm Design}
%\bo{The point of this entire part is unclear, and I do not see how this leads to the next section. The writing also needs to be substantially improved.}
In the following, we also provide useful insights into the design of learning algorithms that can no longer match this lower bound, but also enjoy improved sample efficiency if possible. 
% So far, we have derived a good understanding of the lower bound, yet it is still unclear how to design learning algorithms that can achieve this lower bound.

On the one hand, it is quite straightforward to achieve (nearly) matching upper bound when $\Bex=\wtO(\PTP)$. Specifically, we can ignore all the extra observations and simply employ batched EXP3 algorithm \cite{Dekel2012OnlineBL}, which uses pure bandit feedback only and enjoys a regret of $\wtTheta(\PTP)$.
%\bo{use $\wtTheta$?} \duo{I thought whenever we mention the performance guarantee of an alg. we should use O instead of Theta. Moreover, on some easier instances the regret can be of lower order, so I don't see why use $\Theta$}\bo{we are talking about instance independent bound here, right? Since it achieves the lower bound, it should be fine to use $\wtTheta$}\duo{my point is that, it's not achieving this regret on any instance, but can be smaller. when we say an alg's regret, it's not minimax regret.}
Although the bound matches, per our discussion right after Remark \ref{remark:purdue}, only $\wtTheta(T^{2/3})$ of bandit feedback from all $T$ rounds will contribute to distinguishability due to the tradeoff induced by switching costs, while the rest just become redundant as they do not provide any useful information. Given this observation, it is natural to ask: 
\emph{\textbf{Q1}. Can one still achieve the same regret of $\wtTheta(\PTP)$ while using bandit feedback from $\wtTheta(\PTP)$ rounds only? \textbf{Q2}. Moreover, how would regret scale with the amount of available feedback if the feedback is even more limited (e.g., $\wtO(\PTP)$)?}

On the other hand, it remains largely unknown how to match the lower bound of $\wtOmega(T\sqrt{K/\Bex})$ 
when $\Bex = \wtOmega(\PTP)$. Note that in the derivation of the lower bound, we \emph{optimistically} treat \emph{all} $\Bex$ extra observations as contributing to useful information toward distinguishability (see term~$\mathbf{A.2}$ in \eqnref{extra_lower_bound_before_minimize}). To achieve this, however, one needs to answer an important question: \emph{\textbf{Q3}. How to carefully design a learning algorithm that can properly use these extra observations to indeed gain sufficient useful information toward distinguishability and match the lower bound?}
Furthermore, note that $\Bex = \wtOmega(\PTP)$ and $N_*^s = \wtTheta(\PTP)$.
 %$\Bex = \wtOmega(N_*^s)$.
That is, information obtained from extra observations if all turn out to be useful, would (order-wise) dominate useful information obtained from switching actions (when using pure bandit feedback only). Given this, a further interesting question is: %\textbf{(Q2)} 
\emph{\textbf{Q4}. Can one still match the lower bound of $\wtOmega(T\sqrt{K/\Bex})$ using $\Bex$ extra observations only (i.e., not using any bandit feedback)?}


% \begin{itemize}
%     \item On the one hand, it is quite simple to obtain (near-)optimal upper bound when $\Bex=\wtO(\PTP)$: we can just simply ignore all those extra observations and run batched EXP3 \cite{Dekel2012OnlineBL} which relies on bandit feedback only and enjoys regret bound $\wtO(\PTP)$. Although the bound matches, per our discussion earlier in this section, only $\wtTheta(T^{2/3})$ of bandit feedback from all $T$ rounds will contribute to distinguishability due to the tradeoff caused by switching costs, while the rest just become redundant as they do not provide any information. Given this observation, it is natural to ask: \textbf{Q1.~}\emph{can we still enjoy the $\wtO(\PTP)$ matching upper bound, while we utilize bandit feedback from only $\wtO(\PTP)$ rounds, and hence become more sample-efficient?}
%     \item On the other hand, when $\Bex = \wtOmega(\PTP)$, how to match the $\wtOmega(T\sqrt{K/\Bex})$ is largely unknown. Note that, to get \eqnref{extra_lower_bound_before_minimize}, we \emph{conservatively} assume that \emph{all} $\Bex$ extra observations are transformed into useful ones that provide distinguishability (which is reflected in $\mathbf{A.2}$). However, this is not always the case, i.e., not any arbitrary way to utilize extra observations ensures good exploration, hence we need a careful algorithm design. Moreover, observe that now $\Bex = \wtOmega(\overline{N_*^s})$, i.e., the information collected from switches (namely, bandit feedback) is (order-wise) negligible compared to those extra observations. Motivated by this, we come up with the following question: \textbf{Q2.~}\emph{can we obtain matching upper bound without any bandit feedback (i.e., only relying on $\Bex$ freely-distributed observations)?}
% \end{itemize}

%\duo{rewrite:}

The above questions motivate us to consider a more general setting where the learner has a budget for total observations (Section~\ref{sec:total}). It turns out that the results we obtain for this general setting will also answer the aforementioned questions and lead to learning algorithms that can match the lower bound (up to polylogarithmic factors), hence concluding the minimax regret given in Theorem \ref{thm:bandit_extra_minimax}, along with the lower bound we have shown.


% Motivated by the above questions, we come to realize that the answers to them could be answered and captured as special cases in a more general setting, where the learner makes feedback within \emph{a total budget}. In particular, the answer to $\mathbf{Q1}$ could be viewed as the optimal regret when the learner exploits her total budget (which is no larger than $T$) in a certain way (namely, bandit feedback). And that of $\mathbf{Q2}$ is just a special case when the total budget is $\wtOmega(\PTP)$.


==> sec5.tex <==
\section{Online Learning with Switching Costs and Total Observation Budget}\label{sec:total}

% \xingyu{We may need to divide this section into subsections. Currently, it is too long for this section.}\duo{added three sub-sections}

%In Section~\ref{sec:total}, we aim to understand the role of feedback in this general setting by studying two fundamental questions: \emph{How does regret scale with the amount of all available feedback in general? What is the impact of different types of feedback (bandit, full-information, etc.)?}

In this section, we consider a more general case of online learning with switching costs and a budget for total observations. Specifically, the learner has a budget of $B$ observations, where\footnote{Without loss of generality, we assume $B \geq K$. Otherwise, the learner cannot even observe the loss of some action at least once, thus resulting in linear regret in the worst case.} $B \in [K: KT]$; she can freely choose to observe the loss of up to $K$ actions at each round, as long as the total number of observations over $T$ rounds does not exceed $B$. We aim to understand the role of feedback in this general setting by studying two fundamental questions: \emph{How does regret scale with the amount of available feedback in general? What is the impact of different types of feedback (bandit, full-information, etc.)?}

We first give some additional notations. Let $\mathcal{O}_{t} \subseteq [K]$ be the set of actions whose loss the learner chooses to observe at round $t \in [T]$, and let $N_{ob}$ be the total number of observations, i.e., $N_{ob} :=  \sum_{t=1}^T |\mathcal{O}_{t}|$.
Naturally, we have $N_{ob} \le B \le KT$. For example, bandit feedback is a special case with $\mathcal{O}_{t} = \{X_t\}, \forall t\in[T]$ and $N_{ob} = B = T$; full-information feedback is another special case with $\mathcal{O}_{t} = [K], \forall t\in[T]$ and $N_{ob} = B = KT$.
By slightly abusing the notation in this section, we also use $R^*_T$ to denote the minimax regret over the set of learning algorithms that satisfy the learning protocol specified in Section~\ref{sec:problem setup} and the total observation budget $B$.

\bo{add a brief overview of subsections.}

%Now we sightly abuse the notation and let $\Pi$ denotes the set of all the learning algorithms making $B$ observations in total.
%\bo{Duo, you need to be very careful when addressing comments. There are a lot of editorial issues in your modified test; see this paragraph for example. We may not have enough time.}

\subsection{Minimax Regret and Algorithm Overview}
First, we present a general lower bound under any budget $B \in [K: KT]$ \bo{I do not quite like this notation, which is not straightforward. As long as you make it clear that $B$ is a positive integer, it is fine to use $B \in [K,KT]$}\xingyu{I agree}. This result is stated in \thmref{yasin_lower_bound} below.

\begin{theorem}[Theorem~2 in \citet{seldin2014prediction}]
For any $B \in [K:KT]$, $R_T^*=\Omega(T\sqrt{K/B})$.   \label{thm:yasin_lower_bound}
%$\wtOmega( \frac{T\sqrt{K}}{\sqrt{B}})$.
\end{theorem}

%\bo{Rephrase this paragraph as a remark?}
\begin{remark}
 Note that the above lower bound was originally derived for standard online learning \emph{without} switching costs; it has been shown to be tight (up to a multiplicative $\sqrt{\ln K}$ factor) in the standard setting~\cite{seldin2014prediction}. Clearly, it also serves as a valid lower bound for online learning \emph{with} switching costs we consider. Yet, this lower bound may be loose as introducing switching costs can potentially result in an increased regret rate. A little surprisingly, however, in the sequel we will show that this lower bound is also tight (still up to a $\sqrt{\ln K}$ factor) with switching costs.
\end{remark}

\bo{As I suggested to you, one option is to state the upper bound result in Theorem 3 using $R^*_T$ as well; do not mention any algorithm in Theorem 3. Now, I think we can state Theorem 3 here. Then, you can have a separate subsection focused on the algorithms.}


% \xingyu{rewrite all the parts below until Theorem 3. Please check.}

To enjoy matching upper bound and characterize the minimax regret, we propose an algorithmic framework, of which we will introduce several instantiations later in this section. The complete pseudo-code is given by Algorithm~\ref{alg:framework}.
Overall, our algorithm design takes Online Mirror Descent (OMD) with negative entropy regularizer (also named \emph{Hedge} in the literature) as a sub-routine and runs it over batches, combined with some other techniques (e.g., Shrinking Dartboard~\citep{geulen2010regret}). Before we give a detailed description of our algorithm, let us first highlight its three key components. 

\paragraph{Batching Technique.} We use batching to judiciously distribute the total observation budget $B$. That is, instead of consuming observations at each round as in standard online learning (which in fact may not be feasible when $B$ is relatively small in our case), it only makes observations at a \emph{single} randomly sampled time slot within each batch of rounds. This shares somewhat the same spirit as in~\citet{shi2022power}, although it considers a different problem. 

\paragraph{Shrinking Dartboard (SD).} SD is a celebrated technique to control the expected total number of action switches in online learning by a lazy version of Hedge, i.e., under a carefully chosen probability, the action can remain unchanged across each round~\cite{geulen2010regret} while preserving the same marginal distribution in Hedge. In our algorithm, we generalize this idea to the batching case with general feedback, i.e., the same action can be played across two consecutive batches (rather than rounds) and the full information feedback in~\citet{geulen2010regret} is no longer necessary.

\paragraph{Feedback Obtainment.} Since in our setting, the learner is allowed to freely request feedback within the total budget, our last component lies in feedback obtainment. That is, the learner has the flexibility to determine the loss of which set of actions to observe (not necessarily full information). However, as later we will show, the choice of the observed set could be crucial or even potentially restricted (in some cases) in order to enjoy matching upper bound.

% Therefore, we leave the choice of set $\mathcal{O}_{u_b}$ as a variable component. In fact, 

Now, putting the above three components together, we are ready to present a detailed description of our algorithm below.
In initialization, the algorithm determines learning rate $\eta$, number of batches $N$, batch size $\tau$, and indicator $I_{SD}$ according to $B$, $K$ and $T$. Throughout the game, the algorithm maintains a positive weight $W_b[k]$ for each action $k\in[K]$ at batch $b$. Both the weights and the action for each batch are updated only between two consecutive batches. Hence, in batch $b$, the algorithm keeps playing the determined action $A_b$ until the end of it, and samples a time slot $u_b$ uniformly at random from the current batch and a action set $\mathcal{O}_{u_b}$ in a certain way (to be introduced later) such that the loss of all action(s) in $\mathcal{O}_{u_b}$ at time slot $u_b$ will be revealed to the algorithm. The algorithm then accordingly constructs (unbiased) loss estimate $\widehat{\ell}_b=(\widehat{\ell}_b[1], \dots, \widehat{\ell}_b[K])$ and updates each action's weight by $W_{b+1}[k] \gets W_{b}[k] \cdot \exp(-\eta \cdot \widehat{\ell}_b[k])$. When the indicator $I_{SD}=0$, $p_b$ is always zero, hence the decision $A_b$ is sampled from fresh randomness with probability proportional to each action's weight as Hedge normally does, i.e., $A_b\sim w_b = (w_b[1], \dots, w_b[K])$, where $w_b[k]:=W_b[k]/\sum_{i=1}^K W_b[i]$. Otherwise when $I_{SD}=1$, by the end of each batch, the player is enforced to stay at the current action for the next batch (i.e., $A_{b+1}\gets A_b$) with probability $p_b$, otherwise takes $A_{b+1}\sim w_{b+1}$. 

\begin{algorithm}
    \caption{Batched Online Mirror Descent with Negative Entropy Regularizer and (Optional) Shrinking Dartboard}
    \label{alg:framework}
    \begin{algorithmic}[1]
        \STATE \textbf{Input:} length of time horizon $T$, number of actions $K$, observation budget $B$, batch size $\tau$, number of batches $N=T/\tau$, learning rate $\eta$, and SD indicator $I_{SD}$
        \STATE \textbf{Initialization:} the weight of each action $W_1[k] \gets 1$, and action sampling distribution $w_1[k] \gets 1/K, \forall k \in \left[K\right]$; $\mathcal{O}_t =\emptyset, \forall t\in [T]$ 
        \FOR {batch $b = 1: N$}
            \STATE Sample $u_b$ uniformly from $[(b-1)\tau+1 : b\tau]$
            \STATE Sample action $A_b\sim w_b$ and play this action throughout the current batch, i.e., $X_t = A_b, \forall t \in [(b-1)\tau+1 : b\tau]$\label{lalala}
            \STATE Determine action subset $\mathcal{O}_{u_b}\subseteq[K]$ and observe losses $\{\ell_{u_b}[i]: i\in \mathcal{O}_{u_b}\}$\label{hahaha}
            \STATE Construct (unbiased) estimate $\widehat{\ell}_b$
            \STATE Run OMD update procedure: update action weights $W_{b+1}[k] \gets W_{b}[k] \cdot \exp(-\eta \cdot \widehat{\ell}_b[k])$ and sampling distribution $w_{b+1}[k] \gets \frac{W_{b+1}[k]}{\sum_{i=1}^{K}W_{b+1}[i]}, \forall k\in[K]$
            \STATE $p_b \gets I_{SD} \cdot \exp(-\eta \cdot \widehat{\ell}_b)$
            \STATE With probability $p_b$, stay at the same action, i.e., $A_{b+1} \gets A_b$. Otherwise, sample $A_{b+1}\sim w_{b+1}$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}


% \xingyu{we can put the following part before introducing the algorithm}
% At a high level, the design of our Algorithm~\ref{alg:framework} leverages three main components that will be discussed in detail below. 
% % In particular, in the presence of both switching costs and total budget, we naturally adopt the following three main components in the algorithm design: 

% \xingyu{I will rewrite the following three bullets.}





% batching was originally proposed in \citet{Dekel2012OnlineBL} against \emph{adaptive adversaries} to enjoy desired \emph{policy regret} guarantee while it naturally serves as a technique to achieve low switching, since action switches happen \emph{only between batches} \cite{altschuler2018online}. 
% In this total-budget setting, batching becomes a good fit for designing how to utilize the budget, especially when the budget $B$ is relatively small. (That is, distributing the budget uniformly over all batches.) Moreover, it is very simple to obtain the regret bound of a base algorithm (i.e., sub-routine) after batching through a reduction from the original bound before batching \cite{Dekel2012OnlineBL}.


%The key step to obtain the regret bound after batching is to feed the sub-routine algorithm with the average loss in each batch so that the regret bound after batching can easily be derived through a reduction from the one before batching. Different from \citet{Dekel2012OnlineBL}, our algorithm makes observations in each batch from only one time slot ($u_b$) instead of the whole batch, hence fails to obtain the true batch-average loss and directly apply the original reduction trick in regret analysis, and later we will show that the uniform randomness of $u_b$ turns out to play a key role to tackle this.





% SD first appeared in \citet{cesa2013online} which was used to limit the total number of switches under full information. In particular, for each decision $X_t$, it enforces the algorithm to continue to take the same action for the last decision (i.e., $X_{t-1}$) with probability $\exp(-\eta \cdot \ell_{t-1}[X_{t-1}])$ before directly sampling the action from distribution $w_t$. On the one hand, such enforcement is shown to lead to a tight control on total switches, while on the other hand, it in fact does not change the marginal distribution of action selection, indicating that we still enjoy the same regret guarantee of the original learning algorithm \emph{in expectation}. Although this trick was originally proposed for standard full information setting, it turns out to still play an important role for achieving low switching costs given limited observation budget in some scenarios, hence we use indicator $I_{SD}$ as input to control whether it is applied in our framework.

% \paragraph{Feedback Obtainment.} Since in our setting, the learner is allowed to freely request feedback as long as she is within the total budget, our last component lies in feedback obtainment. That is, the learner has the flexibility to determine the loss of which actions to observe. Therefore, we leave the choice of set $\mathcal{O}_{u_b}$ as a variable component. In fact, as later we will show, the choice of $\mathcal{O}_{u_b}$ could be crucial or even potentially restricted (in some cases) in order to enjoy matching upper bound.


\xingyu{working on the following parts...My general concern is that it does not clearly highlight the type of feedback in the design of algorithm. Also, for the flexible case, Prop. 2 and Prop 3 are quite similar.}\duo{the type lies in the choice of set $\mathcal{O}$.so it's better to merge these two props?}

\xingyu{Here are my initial thoughts that I plan to use to modify the following sections. After stating Thm 3, we turn to discuss the  instantiation. We first say that using full information, we have a universal algorithm for all $B$. Then, just some remarks on further flexible ones. Then, we devote ourselves to discussing the type of feedback, i.e., when $B$ is limited, bandit is sufficient while when $B$ is large, bandit is not sufficient.  }
\bo{I agree. I think that's also what we discussed last week.}\duo{how about now? basically I'll move that part in main body to appendix}

\subsection{The Role of Feedback Amount}

We first show that there indeed exists an instantiation of Algorithm~\ref{alg:framework} that achieves the optimal scaling with respect to the total amount of feedback $B$, i.e., matching the regret lower bound in Theorem~\ref{thm:yasin_lower_bound}, \duo{hence characterizes the role of feedback amount}

% After introducing our algorithmic framework, we formally state its performance guarantee in the following theorem. 

\begin{theorem}
    Given any observation budget $B \in [K:KT]$,
    there exists an instantiation of the algorithmic framework given by \algref{framework} that is able to achieve $\ex{R_T} =  O\left(T\sqrt{\ln K \cdot K/B}\right)$.\label{thm:general_upper_bound}
\end{theorem}

%\bo{I think you want to make it a nice remark here}\duo{like this?$\downarrow$}
\begin{remark}\label{remark:total_budget_minimax_rate}
    Combining the lower bound result in Theorem \ref{thm:yasin_lower_bound} and above upper bound, we can conclude that the optimal minimax rate in this setting is $R_T^* = \wtTheta(T\sqrt{K/B})$ (where $\wtTheta(\cdot)$ hides a $\sqrt{\ln K}$ factor), which is the same as the minimax regret in the setting without switching costs. That is to say, if the learner can freely distribute her observations over all $T$ rounds within the budget, introducing switching costs \emph{does not increase} the intrinsic difficulty of the problem in the minimax sense.
\end{remark}


% It now remains to discuss the specific instantiation of Algorithm~\ref{alg:framework} in Theorem~\ref{thm:general_upper_bound}. To this end, in the following subsections, we first show that there exists an instantiation that can handle all the range of $B$ with 
% In the following two subsections, we first show that there exists a universal 

Note that Theorem \ref{thm:general_upper_bound} does not necessarily give us a uniform algorithm. That is, given different budget $B$, we may need a instantiation with different combination the three components we list earlier. However, we will first provide a uniform but simple algorithm, which can achieve (nearly) matching upper bound for any\footnote{Since we are interested in the asymptotic regret bounds (i.e., both $K$ and $T$ are sufficiently large), we will ignore all the \emph{integrality-related} issues throughout this section. However in Appendix \ref{app:integer} we show how to deal with them while still enjoying the same (asymptotic) regret bound.} $B\in[K:KT]$.


% \subsection{A Simple Yet Uniform Algorithm}
\bo{Check \url{https://www.grammarly.com/blog/capitalization-in-the-titles/} regarding title capitalization rules and follow one style consistently throughout the paper}
In short, our first algorithm is a batched extension of the original SD algorithm \cite{geulen2010regret} with flexible batch size $\tau$ and limited feedback obtainment. In particular, in each batch $b$, our algorithm observes the losses of all $K$ actions at time slot $u_b$. Therefore, the number of batches $N$ should be $B/K$ (since we have $K$ observations in each batch), and batch size $\tau$ is accordingly $T/N=KT/B$.

To obtain the desirable regret guarantee, we need to first show that SD does not change the marginal action sampling distribution, hence it enjoys the same regret bound (without switching costs) from the standard batched OMD. The result is formally stated in \lemref{SD_regret}. Then we can combine it with the standard batching trick to bound the regret . Finally, with \lemref{SD_switch}, all the results altogether imply the desired performance guarantee, which is stated in Proposition \ref{prop:uniform_alg_upper_bound}.

\begin{lemma}\label{lem:SD_regret}
For \algref{framework} with any $\eta>0$, $ \tau\geq 1$, $I_{SD} = 1$, $\mathcal{O}_{u_b}
 = [K]$ and $\widehat{\ell}_b = \ell_{u_b}$  over any loss sequence, we have $\bP\left( A_b = k\right) = \bE[w_b[k]], ~\forall k \in [K] , ~b \in [N]$.
\end{lemma}
\begin{proof}[Proof Sketch of \lemref{SD_regret}]
    The proof mainly follows the original one from \citet{geulen2010regret}, which applies induction to complete the proof. The proof is stated in Appendix \ref{app:SD_regret_proof}.
\end{proof}

\begin{lemma}\label{lem:SD_switch}Running same the instance of \algref{framework} specified in \lemref{SD_regret}, the expected number of switches satisfies that $\bE \left[\sum_{t=1}^T \bI\{X_{t} \neq X_{t-1}\} \right]\leq \eta N = \eta \cdot T/\tau$. 
\end{lemma}

\begin{proof}[Proof Sketch of \lemref{SD_switch}]
    According to the algorithm design, the probability of making a switch between batch $b-1$ and $b$ is at most $1 - p_b$. Therefore, the expected number of total switches could be upper bounded by the sum of those probabilities over all $N$ batches, which completes the proof. We leave the complete proof to Appendix \ref{app:SD_switch_proof}.
\end{proof}

Having both Lemmas \ref{lem:SD_regret} and \ref{lem:SD_switch}, we are ready to formally show its performance guarantee in the following proposition:
\begin{proposition}\label{prop:uniform_alg_upper_bound}
Running \algref{framework} with $I_{SD}=1$, $\eta = \sqrt{\frac{2K\ln K}{3B}}$, $\tau = B/K$, $\mathcal{O}_{u_b} = [K]$ and $\widehat{\ell}_b =\ell_{u_b}$ achieves expected regret $\ex{R_T} = O\left(T\sqrt{\ln K \cdot K/B}\right)$.
\end{proposition}
\begin{proof}[Proof Sketch of Proposition \ref{prop:uniform_alg_upper_bound}]
    The result directly follows \lemref{SD_regret} and \lemref{SD_switch} with the standard reduction trick to show the regret bound after batching from \citet{Dekel2012OnlineBL} and details in Appendix \ref{app:uniform_alg_upper_bound_proof}.
\end{proof}

Although now we have a uniform algorithm to achieve nearly optimal regret (up to a $\sqrt{\ln K}$ factor) for any budget $B$, the way we make feedback is quite restricted: each time we have to observe the losses of \emph{all} actions, which may not be practical or desirable. We may wonder: \emph{can we still enjoy the same regret, while we have the flexibility to decide how many actions to observe each time?}

%The general answer is yes, but we need to deal with two disjoint cases (namely, $B<T$ and $B\geq T$) with some slight difference. Let us use $M\in[K]$ to denote the number of observations we make each time (i.e., $M=|\mathcal{O}_{u_b}|$) and it is not hard to see why $M$ cannot be arbitrary when $B\geq T$ from a simple example: say we have $B=2T$ and $M=1$. In this case, even if we make observation in \emph{all} $T$ rounds, we can only consume $MT=T$, which is just half of the total budget. Hence, for sure we fail to obtain matching regret since we consume only part of the budget. However, such minor issue does not change any fundamental idea behind our algorithm design, and we formally state the flexibility of $M$ in the following propositions:
\duo{The short answer is yes, although it in fact may depend on the value of $B$ and differ a little bit. Let us use $M\in[K]$ to denote the number of observations we make each time (i.e., $M=|\mathcal{O}_{u_b}|$). We formally state the flexibility regarding $M$ in the following proposition. Since there is nothing special in the algorithm design and regret analysis on top of Proposition \ref{prop:uniform_alg_upper_bound}, we leave the detailed discussions and proof to Appendix \ref{app:B<T_upper_bound_proof}.}
\begin{proposition}\label{prop:B<T upper bound}
Running \algref{framework} with $\eta = M\sqrt{\frac{2\ln K}{3KB}}$, $N=B/M$, $\tau = T/N = MT/B$, $\mathcal{O}_{u_b}$ chosen uniformly from $\{S\in 2^{[K]}: |S|=M\}$, $I_{SD}=1$, and $\widehat{\ell}_b[k] = \bI\{k\in \mathcal{O}_{u_b}\} \cdot \frac{\ell_{u_b}[k]}{M/K},\forall k\in[K]$ achieves $\ex{R_T} = O\left( T\sqrt{ \ln{K} \frac{K}{B} } \right)$, where $M$ can be any integer from the set
\begin{equation}
        \left\{
        \begin{aligned}
        [K] & , & \text{given} ~B<T, \\
        [\lceil B/T \rceil:K] & , & \text{given}~ B\geq T.
        \end{aligned}
        \right.
    \end{equation}
\end{proposition}

%\xingyu{the two results are very similar, do we really need to have two separate ones?}\duo{not really. let me see how to merge them two.}
%\begin{proof}[Proof Sketch of Propositions \ref{prop:B<T upper bound}] Propositions \ref{prop:B<T upper bound} further generalizes the proof of Proposition \ref{prop:uniform_alg_upper_bound} from fixed $M$ (which used to be $K$) to a more range in $[K]$. For the complete proofs please see Appendix \ref{app:B<T_upper_bound_proof}.\end{proof}
%In summary, our algorithm design still lies in the spirit of batched SD. However, the flexibility of $M$ differs slightly in two disjoint cases in order to make fully use of the given total budget.
%\begin{remark}Attentive readers may find out that one key step in our proof is to show that $\widehat{\ell}_{u_b}$ is an unbiased estimate of the true average loss for each batch $b$ (namely, $\sum_{i = (b-1)\tau+1}^{b\tau} \ell_{i}/\tau$), which could be viewed as a \emph{sufficient condition}. Following that observation, one may realize that in fact, the losses of actions in set $\mathcal{O}_{u_b}$ do not necessarily come \emph{all from} round $u_b$, but can be from different rounds in batch $b$ \emph{with some uniform randomness which provides unbiasedness}. Such observation provides further flexibility of feedback obtainment for us.\end{remark}

So far, in all the algorithms we have shown, $\mathcal{O}_{u_b}$ comes with some uniform randomness from all action sets with some fixed cardinality $M$, which is definitely valid in our setting. However, this may not be realistic, as in many real-world problems, only the feedback associated with the played action is available and there is no way to observe other actions. Given this practical motivation, it is natural to ask: \emph{what if we exploit the observation budget (which is now no larger than $T$) as bandit feedback only (i.e., $\mathcal{O}_{u_b} = \{A_b\}$)?}

\subsection{The Role of Feedback Type}
Although \citet{Dekel2012OnlineBL} and \citet{dekel2014bandits} altogether imply the $\wtTheta(\PTP)$ optimal regret when $B=T$ under bandit feedback, a tight characterization of the minimax regret for general $B$ is still unclear.

To close this gap, we show another instantiation from our Algorithm \ref{alg:framework}, together with its performance guarantee in the Proposition below.
\begin{proposition}\label{prop:bandit_upper_bound}
Given $B = O(\PTP)$, running \algref{framework} with $\eta = \sqrt{\frac{2\ln K}{BK}}$, $I_{SD} = 0$, $N=B$, $\tau = T/B$ $\mathcal{O}_{u_b}=\{A_b\}$, and $\widehat{\ell}_b[k] = \bI\{k\in \mathcal{O}_{u_b}\} \cdot \frac{\ell_{u_b}[k]}{w_b[k]} $ for any $k\in [K]$ achieves $\ex{R_T} = O\left(T\sqrt{\ln K \cdot K/B}\right)$.
\end{proposition}
\begin{proof}[Proof Sketch of \ref{prop:bandit_upper_bound}]
    The main difference in the proof from previous ones is that, here we directly bounding switching costs by the number of batches instead of using SD.
\end{proof}
In fact, this algorithm can be viewed as a generalization of the original batched EXP3 \citep{Dekel2012OnlineBL} with a flexible batch size $\tau$ and a different way of observing feedback (that is, we only observe one bandit feedback across a batch). One main difference of it from previous algorithms in this paper is that, we are no longer using SD ($I_{SD}=0$) to achieve low switching costs. This is because now the budget is relatively small ($B=O(\PTP)$), and thus bounding switching costs by the number of batches $N$ is sufficient to obtain desired result.

% For sure, our unbiased loss estimate differs a little bit, following the standard construction in adversarial MAB.

Some readers may notice that in Proposition \ref{prop:bandit_upper_bound}, we only consider $B=O(\PTP)$, while leaving $B=\Omega(\PTP)$ alone. However, now we will show how it suffices to show a tight characterization for general $B\in[K:T]$: on the one hand, combining Theorem \ref{thm:yasin_lower_bound} and Proposition \ref{prop:bandit_upper_bound}, we can conclude that given $B=O(\PTP)$, we can still achieve (nearly) matching upper bound in the total-budget setting under bandit feedback. On the other hand, notice that when $B=\Theta(\PTP)$, the optimal regret is $\wtTheta(\PTP)$, which is the same as the one when $B$ is as large as $T$, indicating that even when $B = \Omega(\PTP)$, the optimal regret cannot be improved and remains $\wtTheta(\PTP)$. The intuition behind this has been extensively discussed earlier in Section \ref{sec:extra}, in particular raised in $\mathbf{Q1}$, that is, bandit feedback beyond the quantity of $\wtTheta(\PTP)$ will not provide any useful information in the worst case.

Combining all these cases together, we not only derive a tight characterization between the total observation budget and the corresponding optimal regret, but also state the flexibility of how to make observations, in order to achieve the optimal regret in different scenarios.

Moreover, as mentioned in Section \ref{sec:extra}, now we not only match the lower bound given in Theorem \ref{thm:extra_lower_bound} (up to logarithmic factors) in our first setting, but also answer $\mathbf{Q1}$ and $\mathbf{Q2}$ by getting rid of those redundant feedback which provide no useful information from insights behind both lower bound analysis in Section \ref{sec:extra} and algorithm design in Section \ref{sec:total}.

